Syntactic Language Change in English and German: Metrics, Parsers, and Convergences

Many studies have shown that human languages tend to optimize for lower complexity and increased communication efficiency. Syntactic dependency distance, which measures the linear distance between dependent words, is often considered a key indicator of language processing difficulty and working memory load. The current paper looks at diachronic trends in syntactic language change in both English and German, using corpora of parliamentary debates from the last c. 160 years. We base our observations on five dependency parsers, including the widely used Stanford CoreNLP as well as 4 newer alternatives. Our analysis of syntactic language change goes beyond linear dependency distance and explores 15 metrics relevant to dependency distance minimization (DDM) and/or based on tree graph properties, such as the tree height and degree variance. Even though we have evidence that recent parsers trained on modern treebanks are not heavily affected by data 'noise' such as spelling changes and OCR errors in our historic data, we find that results of syntactic language change are sensitive to the parsers involved, which is a caution against using a single parser for evaluating syntactic language change as done in previous work. We also show that syntactic language change over the time period investigated is largely similar between English and German for the different metrics explored: only 4% of cases we examine yield opposite conclusions regarding upwards and downtrends of syntactic metrics across German and English. We also show that changes in syntactic measures seem to be more frequent at the tails of sentence length distributions. To our best knowledge, ours is the most comprehensive analysis of syntactic language change using modern NLP technology in recent corpora of English and German.

==> abstract_unused.tex <==
\yc{We find indirect evidence supporting \ddm{} for both languages by observing expected diachronic trends in specific measures. However, the most relevant measure, mean dependency distance, is surprisingly increasing over time for German.
%reduced \mdd{} over time is missing for German.
}
%in mean dependency distance, 
%consistent across various parsers and sentence lengths. 
%Three measures consistently exhibit decreasing trends across different parsers and languages, \ab{viz.\ }
\iffalse including \fi
%the left-children ratio, tree degree, and the number of crossing edges.
%Despite \ab{variation} 
\iffalse variations \fi 
%in the trends, the parsers generally show moderate to high agreement with each other. The study also demonstrates that data noise has minimal impact on parser performance, suggesting their effectiveness in parsing text\ab{s} in the 
%\ab{chosen type of corpora.}
\iffalse political debate domain. \fi
Overall, this research sheds light on the diachronic evolution of syntactic features in different languages, offering valuable insights into language change %and optimization trends
\yc{and emphasizing the impact of the parsers on it.}

==> figs/same_length.tex <==
\begin{figure}[!t]
%\vspace{-.5cm}
    \centering
    \begin{subfigure}[]{0.33\linewidth}
        \includegraphics[width=\linewidth]{figs/dec_figs/same_length/mdd.png}
        \vspace{-.6cm}
        \caption{\mdd{}}
        \label{fig:same_len_mdd}
    \end{subfigure}%
    \begin{subfigure}[]{0.33\linewidth}
        \includegraphics[width=\linewidth]{figs/dec_figs/same_length/ndd.png}
        \vspace{-.6cm}
        \caption{\ndd{}}
        \label{fig:same_len_ndd}
    \end{subfigure}%
    \begin{subfigure}[]{0.33\linewidth}
        \includegraphics[width=\linewidth]{figs/dec_figs/same_length/root_distance.png}
        \vspace{-.6cm}
        \caption{\rootdis{}}
        \label{fig:same_len_root}
    \end{subfigure}%
    \quad
    %
    \begin{subfigure}[]{0.33\linewidth}
        \includegraphics[width=\linewidth]{figs/dec_figs/same_length/height.png}
        \vspace{-.6cm}
        \caption{\height{}}
        \label{fig:same_len_height}
    \end{subfigure}%
    \begin{subfigure}[]{0.33\linewidth}
        \includegraphics[width=\linewidth]{figs/dec_figs/same_length/depth_var.png}
        \vspace{-.6cm}
        \caption{\depvar{}}
        \label{fig:same_len_dep_var}
    \end{subfigure}%
    \begin{subfigure}[]{0.33\linewidth}
        \includegraphics[width=\linewidth]{figs/dec_figs/same_length/depth_mean.png}
        \vspace{-.6cm}
        \caption{\depmean{}}
        \label{fig:same_len_dep_mean}
    \end{subfigure}%
    \quad
    %
    \begin{subfigure}[]{0.31\linewidth}
        \includegraphics[width=\linewidth]{figs/dec_figs/same_length/k_ary.png}
        \vspace{-.6cm}
        \caption{\degree{}}
        \label{fig:same_len_degree}
    \end{subfigure}%
    \begin{subfigure}[]{0.33\linewidth}
        \includegraphics[width=\linewidth]{figs/dec_figs/same_length/degree_var.png}
        \vspace{-.6cm}
        \caption{\degvar{}}
        \label{fig:same_len_deg_var}
    \end{subfigure}%
     \begin{subfigure}[]{0.33\linewidth}
        \includegraphics[width=\linewidth]{figs/dec_figs/same_length/degree_mean.png}
        \vspace{-.6cm}
        \caption{\degmean{}}
        \label{fig:same_len_deg_mean}
    \end{subfigure}%
    \caption{Average measures per each of the \emph{Earlier} and \emph{Later} time periods based on dependency relations predicted by Stanza\yc{---Part 1}.}
    \label{fig:same_len_a}
\end{figure}

\begin{figure}[!t]
%\vspace{-.5cm}
    \centering
    \begin{subfigure}[]{0.33\linewidth}
        \includegraphics[width=\linewidth]{figs/dec_figs/same_length/left_child_ratio.png}
        \vspace{-.6cm}
        \caption{\headratio{}}
        \label{fig:same_len_head_ratio}
    \end{subfigure}%
    \begin{subfigure}[]{0.33\linewidth}
        \includegraphics[width=\linewidth]{figs/dec_figs/same_length/topo_edit_distance.png}
        \vspace{-.6cm}
        \caption{\headdis{}}
        \label{fig:same_len_head_distance}
    \end{subfigure}%
    \begin{subfigure}[]{0.33\linewidth}
        \includegraphics[width=\linewidth]{figs/dec_figs/same_length/num_leaves.png}
        \vspace{-.6cm}
        \caption{\leaves{}}
        \label{fig:same_len_leaves}
    \end{subfigure}%
    \quad
    %
    \begin{subfigure}[]{0.33\linewidth}
        \includegraphics[width=\linewidth]{figs/dec_figs/same_length/num_crossing.png}
        \vspace{-.6cm}
        \caption{\crossing{}}
        \label{fig:same_len_crossing}
    \end{subfigure}%
    \begin{subfigure}[]{0.33\linewidth}
        \includegraphics[width=\linewidth]{figs/dec_figs/same_length/longest_path.png}
        \vspace{-.6cm}
        \caption{\lpath{}}
        \label{fig:same_len_path}
    \end{subfigure}%
    \begin{subfigure}[]{0.33\linewidth}
        \includegraphics[width=\linewidth]{figs/dec_figs/same_length/tree_edit_distance.png}
        \vspace{-.6cm}
        \caption{\random{}}
        \label{fig:same_len_random}
    \end{subfigure}%
    \caption{Average measures per each of the \emph{Earlier} and \emph{Later} time periods based on dependency relations predicted by Stanza\yc{---Part 2}.}
    \label{fig:same_len_b}
\end{figure}

==> structure_dec/5_analysis_unused.tex <==


\iffalse
\begin{figure}[!ht]
    \centering
    \includegraphics[width=.6\textwidth]{figs/dec_figs/binsize_hansard.pdf}
    \caption{Spearman correlation between average sentence length per decade and increasing time (decades) for sentences from Hansard within one group. The x-axis denotes the bin size used for grouping, i.e., the difference between the minimal and maximal length in one group. 
    Negative correlations mean that sentence length is decreasing over time and vice versa.
    }
    \label{fig:corr_bin}
\end{figure}
\fi


\section{Analysis}\label{sec:analysis}

\begin{figure}[!ht]
    \centering
    \begin{subfigure}[t]{0.5\linewidth}
        \includegraphics[width=\linewidth]{figs/en_len_dis_random.png}
        \caption{Hansard}
        \label{fig:len_dis_en}
    \end{subfigure}%
    \begin{subfigure}[t]{0.5\linewidth}
        \includegraphics[width=\linewidth]{figs/de_len_dis_random.png}
        \caption{DeuParl}
        \label{fig:len_dis_de}
    \end{subfigure}%
    \caption{
    \yc{Histogram of sentence length distribution}
    %The distribution of sentence length 
    with bin size of 3 
    %\protect\todo{WZ: bin size of 3 means each group contains up to 3 sentences? Better to clarify this.}
    for %the randomly sampled 
    sentences in \texttt{Random} having at most 100 tokens (which compose 99\% of the random dataset). We group the time periods by every 2 decades, except for year 2023, which is merged into the 2000 decade group.}
    \label{fig:len_dis}
    \vspace{-.3cm}
\end{figure}

\todo{SE: a brief summary of what we can expect here}

\subsection{Datasets}\label{sec:datasets}

%show the distribution, average of the sentence lengths and the time periods.

\noindent We apply the preprocessing pipeline introduced in Section \ref{sec:data} to
get up to 200k sentences for each decade and language, and then use the five parsers %above 
\yc{determined in \S\ref{sec:parser}} for parsing. From those sentences, we generate 2 datasets for observation: 
%\begin{itemize}
\paragraph{\textbf{\drandom{}}}
    %\item \textbf{\texttt{Random}}: 
    We randomly sample 2k sentences \fix{longer than 3 words (tokens not tagged as punctuation)} from each decade. The distribution of sentence length is illustrated in Figure \ref{fig:len_dis}. We see a clear trend that there are \fix{more} shorter sentences in the later decades and vice versa; \yc{this is true for both corpora.}
    \ycj{We mainly use this dataset for sanity check instead of exploring syn change.}

%\iffalse
\begin{figure}[!h]
    \centering
    \begin{subfigure}[t]{0.4\linewidth}
        \includegraphics[width=\linewidth]{figs/dec_figs/binsize_hansard_30.pdf}
        \caption{Hansard}
        \label{fig:len_corr_en}
    \end{subfigure}%
    \begin{subfigure}[t]{0.4\linewidth}
        \includegraphics[width=\linewidth]{figs/dec_figs/binsize_deuparl_30.pdf}
        \caption{DeuParl}
        \label{fig:len_corr_de}
    \end{subfigure}%
    \caption{Spearman correlation between average sentence length per decade and time (decades).}
    \label{fig:len_corr}
    \vspace{-.3cm}
\end{figure}
%\fi

\paragraph{\textbf{Effect of grouping sentences by length}}
\yc{\citet{lei2020dependency,liu2022dependency} divide the sentences into groups with 0-10 (0-4 and 5-10), 11-20, 21-30, and 31+ words. In Figure \ref{fig:len_corr}, we demonstrate the Spearman correlation between the average sentence length per decade and decades when applying a similar grouping strategy to our data, which has a difference in length of up to 10 tokens within one group; negative values indicate the average sentence length is decreasing over time. Firstly, for both corpora, %we see that 
the length is strongly negatively correlated to the time for groups having 30+ words %, shown with a correlation ranging from 
(\se{Spearman} $\sim$-0.8 to $\sim$-1). Hence, treating sentences having 30+ words as a single group is not applicable in our case. \todo{SE: not applicable??} 
Secondly, for sentences having less than 30 words,
except for the 0-9 group in Hansard, the other groups also obtain moderate to very high negative correlations ($\sim$-0.5 to $\sim$-1). In contrast, the length of sentences having less than 10 words from Hansard is increasing over time, shown with a positive correlation of $\sim$0.7. 
The reason is that sentences tend to be shorter over time, and consequently, sentences within one group typically have lengths closer to the lower bound for the later periods compared to the earlier periods. 
\todo{SE: (1) I don't understand and (2) the trend is different for English and German} 
Therefore, given the high sensitivity of dependency distance to sentence length \citep{lei2020dependency,zhu2022investigating,zhang2023investigation}, we argue that such grouping is not suitable for observing %the 
diachronic trends of \ddm{}-related metrics, at least for our data. This may also cast some doubts on the findings of previous approaches that do not consider a more fine-grained grouping or do not compare sentences of exactly the same length, because it is possible that the observed (up)downtrend of dependency distance results from the trend of sentence length over time instead of the real language change.}


\paragraph{\textbf{\texttt{Balance}}}
\yc{Being aware of the above, we carefully construct a balanced dataset, eliminating the correlation between sentence length and time. 
%To ensure sufficient sentences for different lengths and time period, we group every two decades together and 
We build sentence groups for lengths in [5, 10, 15, 20, 30, 40, 50, 60, 70] with a maximal difference of 3 tokens in sentence length within one group. 
\todo{SE: basically, you reduce the width of the interval/bin, right?}
E.g., in the group for length 10, sentence length ranges from 10 to 12. To ensure a sufficient amount of sentences for each length group and time period, we randomly sample 450 sentences for every two decades (with 2020 as an exception, which is merged into the 2000-2010 decades). \todo{SE: 2020 should go to 2010-2020, right?}
Our final dataset contains $\sim$1905 sentences per decade for German 
    ($= 450 \times 9 \text{ length groups} \times 8 \text{ decade groups} \div 17 \text{ decades}$) %$\approx$ 1905) 
    and $\sim$1937 sentences per decade for English ($= 450 \times 9 \text{ length groups} \times 11 \text{ decade groups} \div 23 \text{ decades}$).}
    
    %\item \textbf{\texttt{Balance}}: 
    \iffalse
    Since sentence length plays a great role in metrics like dependency distance \citep{lei2020dependency,zhu2022investigating,zhang2023investigation},
    \fix{we carefully group the sentences so that there is no tendency for sentences to be shorter in the later time periods within a group.  
    %\todo[inline]{WZ: not clear. You mean each decade-group contains the same amount of sentences with similar sentence lengths through sampling? What is the optimal bin size? So, bin size controls the number of sentences in each group; length group controls the sentence lengths of each group? Actually this paragraph is quite difficult to understand. Why sentence length per decade is decreasing over time, given that "no tendency for sentences to be shorter in the later periods".}
    Firstly, we inspect the optimal bin size for sentence grouping. To do so, we select the anchor length [0, 10, 15, 20, 30, 40, 50, 60, 70] for length groups and the bin size (i.e., the difference between the minimal and maximal length in one group) of 0 to 10. 
    For instance, sentences in the group with an anchor length of 10 and bin size of 5 have 10-14 tokens. Then, we calculate Spearman's $\rho$ correlation \citep{spearman1961proof} between the average sentence length per decade and the %time series (here we use 
    decades in ascending order for each anchor length; negative correlation implies that the average sentence length per decade is decreasing over time within a group 
    and vice versa. As Figure \ref{fig:corr_bin} \ab{shows}, except for the group of the anchor length 0, where the correlation raises to above 0.6 with increasing bin size, the correlations for all other groups decline to nearly -1 when \ab{the} bin size \ab{is} $10$, which suggests a strong negative correlation between sentence length and time. Hence, we argue that the grouping strategy  
    in \citet{lei2020dependency,liu2022dependency} does not suit our data (at least), \yc{which %coarsely 
    grouped sentences 
    having $\leq$ 30 words with a bin size of 10 (and/or 5), while treating sentences with more than 30 words as a single group.}
    \yc{We randomly sample 450 sentences for every two decades, and limit the maximal }
    }\fi
    %\todo{YC: for some reason I could not reproduce the previous result anymore, maybe I made a mistake. The sampling of the 450 sentences seems to play a greater role in balancing compared to the bin size. Need to complete this. SE: what can you not reproduce?}

    %\todo{SE: do not understand `which coarsely group [...]' until end. I guess, it's ungrammatical, too}
    
    \iffalse
    %we carefully create a balanced dataset across sentence lengths. 
    The sentence length is calculated as 
    %We treat 
    the number of tokens in sentences tokenized by Stanza.
    %as the sentence length.
    To ensure sufficient sentences for each length group and time period, we group every two decades together (with 2020 as an exception, which is grouped into the 2000 decade group), and select 450 sentences for each of the %with 
    anchor lengths [5, 10, 15, 20, 30, 40, 50, 60, 70] %for each 
    per decade group. The balanced dataset has $\sim$1905 sentences per decade for German 
    (450 $\times$ 9 length groups $\times$ 8 decade groups $\div$ 17 decades $\approx$ 1905) and $\sim$1937 sentences per decade for English.
    %$\div$ 2 decades $\approx$ 2k sentences per decade). 
    In our initial experiment, we grouped sentences in bins of size \fix{10, following \citet{lei2020dependency,liu2022dependency}; for example, sentences of lengths 20-29 were placed in the group of anchor length 20
    Nevertheless, such a grouping strategy leads to unbalanced data because the earlier decade groups tended to have \fix{more} longer sentences of lengths close to the upper bound and vice versa%of length close to the %anchor length
    %upperbound
    ---the mean sentence length in the resulting dataset is consequently decreasing over time and 
    that of decade group 2000 is 5 
    %times smaller 
    tokens less than that of group 1860 for German, for example. \todo{YC: I could not reproduce this result anymore, maybe I made a mistake. Need to change this. The sampling of the 450 sentences seems to play a greater role in balancing compared to the bin size.}
    Thus, we restrict the bin size to 3 for length grouping; the final dataset has differences of less than 0.1 in mean sentence length across decade groups.}
    Thus, we restrict the bin size to 3 for length grouping; the final dataset has differences of less than 0.1 in mean sentence length across decade groups.
    \fi
    %, and no downtrend 
    %for both English and German.  
%\end{itemize}
%(1) We randomly sample 2k sentences from each decade, denoted as \textit{Random}. (2) We use ChatGPT to filter out non-sentence texts and also let ChatGPT correct the sentences for German; 2k random sentences curated by ChatGPT are retained per decade for both languages (denoted as \textit{ChatRandom}). (3) Since %many works have shown that 
%sentence length plays a great role in metrics like dependency distance \citep{lei2020dependency,zhu2022investigating,zhang2023investigation}, we create a fully balanced dataset across sentence lengths. To ensure sufficient sentences for each length group and time period, we group every two decades together and select sentences with anchor lengths [5, 10, 15, 20, 30, 40, 50, 60, 70] for each decade group. In our initial experiment, we group sentences in bins of size 5; for example, sentences with lengths of 20-24 are placed in one length group. However, such grouping strategy still led to unbalanced data because 




\subsection{Trend Test}

Following \citet{zhu2022investigating,liu2022dependency}, %\todo{add citation}
we perform the Mann Kendall (MK) trend test \citep{mann1945nonparametric} to indicate the diachronic change of the concerned metrics. 
%Mann Kendall  
\se{MK}
trend test is widely used to detect trends in %the 
time series. Additionally, 
%as some measures are obviously highly correlated to %the 
%sentence length, such as the tree height and root distance, 
\yc{because of the high sensitivity of \ddm{} metrics to sentence length,}
we perform \yc{an extension} of MK, namely the partial Mann Kendall (PMK) test \citep{libiseller2002performance}, which 
\yc{can effectively distinguish
%reduce the influence of 
non-meaningful changes 
%on the trend of 
from time series data. In our case, the changes in metrics resulting from sentence length changes
%the influence of sentence length 
should be considered non-meaningful.}
%reduces the influence of other independent variables on the response variable by considering the conditional distribution of the MK statistics.
%\todo[inline]{WZ: High correlation between sentence length and measures is problematic or not? Why this is the reason for adopting PMK test? About the last sentence "reduces the influence..", what you want to say...} 
%In our case, we perform the PMK trend test for the measures %in the presence 
%\yc{with awareness}
%of the sentence length.
%\todo[inline]{WZ: "in the presence of sentence length"---what do you mean by that..} 
For both trend tests, we use the implementation from \citet{Hussain2019pyMannKendall}.\footnote{\url{https://github.com/mmhs013/pyMannKendall}}






%\paragraph{\textbf{}}
\input{tables/trendtable}
\subsection{Results}
%\todo[inline]{WZ: these results are based on the random or balanced datasets?}

\subsubsection{Impact of parser selection}\label{sec:anaysis_agree}
%\vspace{1cm}\noindent\textbf{RQ2: \emph{Do dependency parsers agree with each other?}}\\

\noindent 
\yc{As the other relevant approaches rely on a single parser, we first investigate whether different parsers yield the same outcomes in terms of trend tests.}
The trend tests have three outputs: ``no trend'', ``decreasing'', and ``increasing'', which can be seen as the labels of 
a three-way classification task.
%we first investigate the impact of using different parsers on the diachronic trend analysis. %\todo[inline]{WZ: perhaps adding a sentence to explain why you change the correlation measure to Cohen's Kappa?}
%To do so, 
Therefore, we calculate %the 
Cohen's Kappa %agreement 
between %the %results of 
the trend test results based on different parsers. \yc{Low agreement may indicate limited robustness in observations relying on one parser.}
We use all trend test outputs on the \texttt{Random} and \texttt{Balance} datasets, resulting in 
\fix{330  test cases ($=$ 2 trend tests $\times$ 15 measures $\times$ (1 trend on \texttt{Random} + 1 overall trend on \texttt{Balance} + 9 trends on \texttt{Balance} for different sentence length groups))} for each %parser and 
language. %(2 trend tests $\times$ 15 measures $\times$ (1 trend on \texttt{Random} + 1 overall trend on \texttt{Balance} + 9 trends on \texttt{Balance} for different sentence length groups) = 330). 
We then calculate the agreement on the 330 trends between the parsers. 

%\todo{SE: symmetric matrix --- only keep half of entries YC: We have enough space anyway. the page limit is 15-25. I prefer to keep it.}

\begin{figure}[!ht]
\vspace{-.5cm}
    \centering
    \begin{subfigure}[t]{0.45\linewidth}
        %\includegraphics[width=\linewidth]{figs/hansard_parser_corr_all.png}
        \includegraphics[width=\linewidth]{figs/dec_figs/corr_triangle_en.pdf}%{figs/dec_figs/hansard_parser_corr_no_aggreg.png}
        \caption{Hansard}
        \label{fig:parser_cor_en}
    \end{subfigure}%\hspace{-.3cm}
    \begin{subfigure}[t]{0.45\linewidth}
        %\includegraphics[width=\linewidth]{figs/deuparl_parser_corr_all.png}
        \includegraphics[width=\linewidth]{figs/dec_figs/corr_triangle_de.pdf}%{figs/dec_figs/deuparl_parser_corr_no_aggreg.png}
        \caption{DeuParl}
        \label{fig:parser_cor_de}
    \end{subfigure}%
    \caption{Cohen's Kappa between the results of %the original and partial Mann Kendall trend test 
    MK+PMK tests based on the dependency relations predicted by different parsers. Deeper colors denote higher agreement and vice versa. We show the average agreement for each parser in the \yc{first} row.}
    \label{fig:parser_cor}
    \vspace{-.3cm}
\end{figure}

We show the agreement matrix in Figure \ref{fig:parser_cor}. Most parsers demonstrate a moderate to high agreement with others (0.6-0.8). On \textbf{English} data, as illustrated in Figure \ref{fig:parser_cor_en}, the highest agreement of \fix{0.88} is observed between Stanza and StackPointer, succeeded by Stanza and Biaffine (0.78); Stanza obtains the highest average agreement with others (0.74), followed by \fix{Biaffine and StackPointer (0.7). The three of them also obtain a relatively high agreement with each other (0.72-0.88), in contrast to their agreements with the others (0.54-0.69).
Among the parser pairs, CoreNLP and StackPointer obtain the lowest agreement of 0.45. %---we then observe that
%all parsers achieve their lowest agreement with CoreNLP, compared to their agreements with other parsers
%(0.47-0.56 vs. 0.53-0.85). 
%Besides, we note that 
TowerParse and CoreNLP %also 
exhibit %a relatively 
the lowest average agreement with others (0.57 and 0.61 respectively).
%, especially with StackPointer (0.53) and CoreNLP (0.50).
}
As for \textbf{German} (Figure \ref{fig:parser_cor_de}), similarly, the highest agreement is \fix{achieved between Stanza and StackPointer (0.78), followed by StackPointer and Biaffine (0.76); 
Stanza also obtains the highest average agreement (0.69), while CoreNLP least agrees with others (0.45-0.57). 
%, and between StackPointer and Stanza (0.77). Again, the lowest agreement is found between CoreNLP and StackPointer (0.45) and this low agreement with CoreNLP is consistent across parsers, ranging from 0.45 to 0.59. Similar to the observation on English data, %to the English data, 
%Stanza achieves the highest average agreement (0.7), followed by Biaffine and StackPointer (0.67-0.68), and these three parsers %also
%exhibit a higher level of agreement with each other (0.76-0.77), compared to their agreement with other parsers, which falls within the range of 0.45-0.67.
} 

\vspace{-.2cm}
\paragraph{\textbf{Takeaway}}
In summary, our observations indicate that for both languages, \textbf{\emph{the use of different parsers may 
lead to various conclusions about
diachronic %trend of 
syntactic changes \yc{regarding \ddm{}}}}.
%the parsers do not always agree with each other.
%(1) Stanza exhibits the highest agreement with other parsers, while (2) CoreNLP demonstrates the lowest agreement; and (3) Biaffine, StackPointer, and Stanza agree with each other more than with other parsers. 
This raises %some 
concerns about previous approaches %that conclude their findings 
%with heavy reliance 
\se{which heavily rely} 
on the CoreNLP parser, which 
exhibits the lowest agreements with other parsers in our experiment.

\input{figs/same_length}

%\vspace{1cm}\noindent\textbf{RQ3 \& RQ4: \emph{Which measures are decreasing/increasing over time? Do they show the same trend in English and German?}}\\

\subsubsection{Diachronic \se{syntactic} language change}\label{sec:analysis_change}
\noindent \yc{We base our observations on both \drandom{} and \balance{} datasets. Following \citet{juzek2020exploring,krielke2023optimizing,zhu2022investigating}, we compare %the 
sentences %having at most 70 tokens 
of identical length, leveraging the \textbf{\drandom{}} dataset. \todo{SE: what about binning?} 
We also perform the trend tests%using our \textbf{\balance{}} dataset
, following \citet{zhu2022investigating,liu2022dependency}, to minimize the effect of sentence length here, we use our \textbf{\balance{}} dataset.} \todo{SE: make two sentences??}

\fix{
\paragraph{\textbf{\texttt{Random}}}
%Following \citet{juzek2020exploring,krielke2023optimizing}, we first inspect the syntactic shifts on sentences of exactly the same length, using the Stanza parser, given its highest agreement with others. \todo[inline]{WZ: what are the results of your inspection on syntactic changes?}
%and the \texttt{Random} dataset. 
\yc{
We use the parsing results from Stanza, since it obtains the highest agreement with other parsers. 
%We limit the sentences to those having at most 72 tokens and 
We only %coarsely 
divide the data into two time periods, \emph{``Earlier''} and \emph{``Later''}, 
%as there are too few longer ones in our data. 
to get more sentences for each length;}
%Here, we only %coarsely 
%divide the data into two time periods, \emph{``Earlier''} and \emph{``Later''}, to get more
%sufficient amounts of 
%sentences for each length; 
this helps reduce the impact of outliers. 
Additionally, we limit the sentences to those having $\leq$72 tokens to %keep 
\se{be} 
consistent with the \texttt{Balance} dataset. 
%the same purpose.
%For the \textbf{English} data, the \emph{Earlier} period is from decade 1800 to 1900 and the \emph{Later} from 1910 to 2020; 1860-1940 is treated as the \emph{Earlier} period and 1950-2020 the \emph{Later} period for \textbf{German}. %The resulting data has 
In the case of \textbf{English} data, the Earlier period spans from the decade 1800 to 1900, and the Later period ranges from 1910 to 2020. For \textbf{German}, the Earlier period is defined as 1860-1940, while the Later period is from 1950 to 2020.
}

\todo{SE: based on which parsers? why do we see our results confirmed? Just because it's randomly shuffled?}

\fix{We demonstrate the metrics on the sentences in both languages of identical length in Figure \ref{fig:same_len_a} and \ref{fig:same_len_b}. %We observe that: (1) 
Firstly, %we see that 
%regarding our main interest, \textbf{\mdd{}}, 
\yc{regarding the comparison between English and German, the observations meet 7/9 of our expectations: German has a larger \mdd{}, \crossing{}, \degvar{}, \degree{} and \headratio{}, as well as a smaller \headdis{} and \height{}, compared to English; the 2 exceptions are \ndd{} and \leaves{}. Besides, we also see that German has a smaller \depvar{}, \depmean{} and a larger \lpath{} than English; the \degmean{}, \leaves{} and \random{} for the two languages are almost the same.}
%among our hypotheses for the comparison between German and English, 
%we see that German sentences have larger \mdd{} than English (Figure \ref{fig:same_len_mdd}), which is consistent with \yc{our expectation} and the previous finding that German has been less optimized in terms of \ddm{} \citep{gildea2010grammars,ferrer2022optimality}; 
For \textbf{English}, we do not see a clear difference in \mdd{} between the two periods for sentences with less than 50 tokens; however, sentences having more than 50 tokens often have a smaller \mdd{} for the \emph{Later} period than for the \emph{Earlier} period.  
Furthermore, we observe a general increase in \height{}, \depvar{} and \depmean{}, and a decrease in \degree{}, \degvar{} and \headratio{}, for English sentences having more than 30 tokens.
Counter-intuitively, %the line plots suggest that 
%the 
\mdd{} for \textbf{German} is even larger in the \emph{Later} period compared to the \emph{Earlier} period; %\todo{SE: but in both cases not by much}
%As 
 %For \textbf{German}, %an increase in 
while \rootdis{}, \depmean{} and \lpath{} are found to be larger in the \emph{Later} period, \degree{}, \degvar{} and \headratio{} become smaller, for most lengths.  
}
%\todo{SE: in accordance with our hypotheses or not?}

%\todo{SE: Fig 12+13 have identical captions?}


\paragraph{\textbf{\texttt{Balance}}}
%Next, r
Recognizing that different parsers can lead to varying %conclusions in 
trends, %tests, 
we employ a majority vote approach to identify the stable trends across parsers, i.e., if at least 3 out of 5 parsers agree on a trend, we consider it 
%a 
stable. %\todo{SE: why only for Balance?}
%trend. 
%This method aims to identify consistent trends across parsers. 
Besides, observing that the outcomes of the two trend tests often differ from each other, %especially on the \texttt{Random} datasets, 
%\todo{SE: why? because the trends are strong ones?}
we further restrict the valid trends to those being consistent across the two trend tests. Here, we perform the trend tests on the \texttt{Balance} dataset, \fix{since those metrics are very sensitive to the sentence length, as shown in Figure \ref{fig:same_len_a} and \ref{fig:same_len_b}.}

We present the results of the trend tests in Table \ref{tab:trend}, which shows %the 
consistent trends across tests that are agreed by at least 3 parsers, except for \#Crossing, for which we relax the minimal requirement to 2 parsers, as CoreNLP cannot predict %the 
non-projective relations. ``$+$'' and ``$-$'' before the numbers denote %the 
increasing and descreasing trend\se{s}, repectively\se{,} and the values after ``$+$/$-$'' refer to the number of parsers that support %in 
this trend. \todo{SE: support in this trend?}

As shown in Table \ref{tab:trend}, on the \textbf{\texttt{Balance}} dataset: %we observe that:
 overall, (1) in \textbf{English}, we observe an \emph{increase} in the \height{}, \degmean{}, \depmean{} and \depvar{} 
 %are \emph{increasing}
 over time, while the \mdd{}, \headratio{}, \degree{}, \rootdis{} and \crossing{} are \emph{decreasing};
 %over time; 
 (2) in \textbf{German}, the \mdd{}, \lpath{} are \emph{increasing} over time, whereas the \ndd{}, \headratio{}, \degree{}, \leaves{}, \degvar{}, and \crossing{} demonstrate a \emph{downward} trend. 
  We find three metrics that show downtrend in both languages, i.e., the \headratio{}, \degree{}, as well as the \crossing{}. 
 All of the other metrics show different trends across languages, including \mdd{}, which has been shown to be decreasing over time in English in previous work \fix{(e.g., \citet{lei2020dependency})}. %\todo{add citation}
%It is worth noting that in German, 
We also see a downward trend of \mdd{} in English, especially for sentences of length greater than 30, where in 4 out of 5 length groups, 3-5 parsers support the decreasing trend. However, %we do not see a clear %clue about the 
\se{there is no clear} 
trend in sentences of length smaller than 30. In contrast, we observe a consistent uptrend in \mdd{} in German across different sentence lengths: in 7 out of 9 length groups, this trend is confirmed by at least 4 parsers. %As for NDD, we see an anti-minimization 
\ndd{}, as the normalized version of \mdd{}, is expected to demonstrate a consistent trend with \mdd{}; %on the balanced dataset across sentence lengths; 
however, it suggests a totally opposite direction than \mdd{} %with respect to
for the \fix{diachronic} change in German, where \mdd{} is increasing while \ndd{} \ab{decreases} over time. We note that in \citet{zhang2023investigation}, the \mdd{} and \ndd{} for the English news text\ab{s} also demonstrate inconsistent trends, where \mdd{} gradually \ab{increases} over time, while \ndd{} does not show any clear trend. 
Those may cast doubts on the legitimacy of the \ndd{} metric, \fix{especially for languages other than English.}

\fix{%trends are different for different lengths\\
%For many measures, we observe different trends for shorter and longer sentences. 
%varying length groups. 
While direct evidence for anti-\ddm{} is missing, given the limited significance of \ddm{} in our observations, we often see distinct trends of many other metrics between short and long sentences, such as the \degree{}, \depmean{}, and \headratio{} of both English and German sentences. This may imply that language optimization %processes may 
indeed predominantly impact\se{s} long sentences. %\todo{SE: lang opt predominantly affects sentence length?}
%we see reverse trends of short sentences 
%Similar to the anti-\ddm{} phenomenon, many measures show varying diachronic trends for shorter and longer sentences. Despite   
%Being aware of the existence of anti-\ddm{} phenomenon,
}

\todo{SE: the last paragraph leaves me confused. It's too much to understand what's going on (parsers, measures, languages, ...)}

\paragraph{\textbf{Takeaway}}
\fix{Despite lacking direct %clue 
\se{evidence}
of \ddm{} \yc{from \mdd{} and \ndd{}} in our observations, the trends of other relevant measures seem to support it. % strongly. \todo{SE: a bit out of the blue. not mentioned above??}
Due to the pressure of \ddm{},
%hierarchical structures of the dependency trees are preferred, and thus, 
some specific trends of measures are expected based on established linguistic studies (%as mentioned in
see \S\ref{sec:measure})% to reduce the probabilities of long dependency distance
: (1) decreasing \degvar{}, to de-centralize the heads in dependency trees; (2) increasing \height{}, for enlarging the hierarchical levels of dependency trees; (3) decreasing \headratio{} and increasing \headdis{}, to reduce the head-final cases; (4) decreasing \crossing{}, as %the 
\se{a}
side-effect of \ddm{}. All of those trends have been observed for both languages in our experiments, especially for the longer sentences; however, they are less prominent for the short sentences. 
Therefore, our findings overall provide indirect evidence of \ddm{} and anti-\ddm{} in short sentences, \todo{SE: What??}
from a diachronic perspective. 
%our findings still support the syntactic language change in terms of \ddm{} and also . 
}
%\todo[inline]{WZ: what are the implications of these results on syntactic changes? Did you cross-check the results on random and balanced datasets; any commonalities and differences?}

%\todo{SE: is that the takeaway?}

%\todo{SE: Fig.12+13 not properly discussed, are they? Are trends strong or mild? Can we give illustrations of those trends? Why only stanza? Btw. why did we go to two cases (earlier vs. later only) instead of fine-grained trend analysis?}

%\todo{add examples for each measure}


==> structure_dec/8_ack.tex <==
%\clearpage
\section{Acknowledgement}
blabla

==> structure_unused/1_intro.tex <==
\section{Introduction}

\begin{figure}[h]
    \centering
    \includegraphics[width=.67\textwidth]{figs/intro_linear.pdf}
    \includegraphics[width=.31\textwidth]{figs/intro_tree.pdf}
    \caption{Dependency relations of sentence ``%
    %I see no reason for altering the form.
    \fix{But there is no proof.}'' in linear order (left) and tree graph (right).}
    \label{fig:intro}
\end{figure}
\todo{replace with/add an overview figure; redo the fig with tikz}

Many studies have shown that human languages are being optimized \ab{over time} towards lower complexity and higher efficiency in terms of communication \citep{gibson2019efficiency,ferrer2022optimality,degaetano2022toward}.
%[Gibson et al., 2019; Ferrer-i-Cancho 2022; Degaetano-Ortlieb, and Teich 2019]. 
Among others, syntactic dependency distance, i.e., the linear distance between syntactically dependent words, is often perceived as the indicator of language processing difficulty and working memory load of humans.\citep{temperley2007minimization,liu2008dependency,zhu2022investigating,juzek2020exploring}.
%[Temperley, 2007; Liu, 2008; Liu et al., 2017; Zhu et al. 2022; Juzek et al. 2020]. 
The corresponding optimization principle is well-established,  i.e., dependency distance minimization (DDM), which refers to the tendency/preference of syntactically related words being placed closer to each other.

A large array of works have confirmed the existence of DDM in natural languages (e.g., \citet{temperley2007minimization,futrell2015large,juzek2020exploring,zhang-etal-2020-efficient}).
%[Temperley, 2007; Furtrell et al., 2015; Juzek et al., 2020; Zhang and Zhou, 2023]. 
On the one hand, studies suggest that the mean dependency distance (or its variant) of a real sentence is shorter than that of the random baselines (e.g., the sentence with random word orders) and this may be a universal property of most natural languages \citep{gildea2010grammars,futrell2015large,ferrer2022optimality}.
%[Gildea and Temperly, 2010; Furtrell et al., 2015; Ferrer-i-Cancho et al., 2022]. 
On the other hand, there is also evidence of DDM found in the diachronic investigations of (English) language change, i.e., the mean dependency distance is decreasing over time \citep{lei2020dependency,liu2022dependency,juzek2020exploring,zhang2023investigation,zhu2022investigating}.
%[Lei and Wen., 2020; Liu et al., 2022; Juzek et al., 2020; Zhang and Zhou, 2023; Zhu et al., 2022]. 
However, no such research exists for languages other than English.
%\emph{it is still unanswered whether the trend of diachronic DDm is generalizable to other languages}. 
In this work, we go one step further and explore the diachronic trend of DDM in both English and German, aiming to answer the question \emph{whether this trend is generalizable to other languages} (Section \ref{sec:analysis}). 

Such diachronic investigation involves using dependency parsers to automatically parse the syntactic structure of the sentences from a corpus covering a large time span and then making observations on the parsed dependency structures. To our best knowledge, all of the previous works \citep{lei2020dependency,juzek2020exploring,zhu2022investigating,zhang2023investigation,liu2022dependency} leveraged the Stanford CoreNLP parser \citep{manning-etal-2014-stanford}, which was published nearly 9 years ago. \citet{lei2020dependency} show that the errors stemming from the parsers do not affect the final results substantially. They manually corrected the parsing outputs and computed the correlation between the measures on the original and on the corrected dependency relations. Nevertheless, we argue that such a correction procedure may introduce bias since humans are exposed to the solution from the parser when making decisions. Besides, we are also interested in \emph{whether those observations are stable across different parsers}.
Hence, in this work, we rely on 5 dependency parsers, including CoreNLP and 4 newer ones, to make observations and investigate to what extent the parsers agree with each other, in terms of the detected diachronic trend resulting from their parsing outputs (Section \ref{sec:analysis}).

Besides, those parsers are mostly trained and evaluated on modern treebanks, which cover a small time span compared to those diachronic corpora. Thus,
we also examine \emph{the potential noise in the corpora and assess its impact on the parsers' performance} (Section \ref{sec:parser}).

%Besides the 
Dependency relations can also be structured as a rooted directed tree, as shown in Figure \ref{fig:intro} (right). %\todo{add a tree graph}
Therefore, measures beyond linear dependency distance %are able to 
can be explored. Unlike the other works that only focus on the dependency distance, in this work, we \emph{quantitatively analyze the diachronic trend of 15 measures in total}, including the dependency distance and others based on the properties of the tree graphs, such as the tree height and degree variance (Section \ref{sec:analysis}). 

Our contributions are:
\begin{itemize}
    \item We explore: (i) how the 15 measures including the mean dependency distance are changing over time, in both English and German, using two extensive corpora containing texts in the political debate domain; (ii) whether those diachronic trends are consistent across different parsers and languages; (iii) how the dependency parsers perform on the diachronic corpora in the political debate domain. %(iv) which types of noise exist in those corpora. 
    
    \item We show: (iv) in contrast to English, German demonstrates an uptrend of the mean dependency distance; this finding is consistent across different parsers and sentence lengths; (v) three measures demonstrate consistent trends across different parsers and languages, i.e., the downward trend of left-children ratio, tree degree, and number of crossing edges (Table \ref{tab:trend}); (vi)
    the parsers do not always agree with each other in terms of the trend test results, mostly obtaining a moderate to high agreement. (vii) the data noise does not substantially affect the parsers' performance and those parsers are able to parse the text in the political debate genre. 
    %\item 
\end{itemize}

%Dependency distance  

%Furtrell et al., 2015; Ferrer-i-Cancho et al., 2022 compared DDm across 37/97 languages from varying linguistic families and showed that the degrees of DDm indeed vary for different languages; however, their comparison was limited to a synchronic scope as the used treebanks only contain the data for a small time span. Gildea and Temperly, 2010 observed that DDm has a much weaker impact on German than on English, also from a synchronic perspective. Lei and Wen., 2020; Liu et al., 2022; Juzek et al., 2020; Zhu et al., 2022; Zhang and Zhou, 2023 analyzed dependency distance based on diachronic corpora covering large time spans, but all explored corpora are for English. Moreover, all of the mentioned diachronic investigations leveraged the Stanford CoreNLP parser, which was not specifically trained and evaluated on historical data; therefore, it may have led to biased conclusions, as a consequence of incorrect parsing. Furthermore, DDm has been identified as the origination of other manifestations of syntactic structure optimizations, such as the scarcity of crossing dependencies (Gómez-Rodríguez and Ferrer-i-Cancho, 2017; Ferrer-i-Cancho and Carlos Gómez-Rodríguez, 2021), and can even predict other principles of language optimization beyond syntax like the minimization of word lengths (Ferrer-i-Cancho and Carlos Gómez-Rodríguez, 2021); these highlight the importance of studying DDm for understanding language change. 





==> structure_unused/2_related.tex <==
\section{Related Work}

\fix{This work connects to dependency distance minimization (\ddm) and language change.}

\paragraph{\textbf{Language Change}}

%\paragraph{\textbf{Syntactic Language Change}}
\paragraph{\textbf{Dependency Distance Minimization}}
\fix{The most relevant approaches to ours are those based on sentential dependency structures, where (a.o.) the dependency distance and the corresponding principle (i.e., DDM) %, %i.e., the linear distance between two syntactically dependent words within a sentence \citep{hudson2010introduction,tesniere2015elements,lei2020dependency}, 
have been researched extensively. %from both synchronic and diachronic perspectives. 
%On the one hand, 
From a \textbf{synchronic} perspective, many studies have shown that the mean dependency distance (\mdd) (or its variant) of a real sentence is shorter than that of some random baselines (e.g., the sentence with random word orders). %, from a \emph{synchronic} perspective. 
For example, \citet{FerreriCancho2004EuclideanDB} and \citet{liu2007probability} observed that the mean dependency distance of Romanian/Czech and Chinese sentences is significantly shorter than that of random sentences, respectively.
\citet{liu2008dependency,futrell2015large} %investigated DDM in 37 languages. They 
provided %the %first 
large-scale evidence of DDM%based on cross-lingual studies
, which suggests that DDM may be a universal property of human languages. They used treebanks %the dependency-annotated corpora 
of %37 
different languages from various linguistic families to perform the tests 
and showed that the dependency distance of real sentences is shorter than chance. %; this indicates that human languages indeed have undergone optimization due to the pressure of DDM. 
More recently, \citet{ferrer2022optimality} analyzed the optimality (based on dependency distance) of 93 languages from 19 linguistic families. %They defined a new metric that can measure the optimality of a certain language and the resulting cognitive pressure based on the dependency distance. 
Their results imply that 50\% of human languages have been optimized to a level of at least 70\%. Compared to English, %which obtains an optimality score of 0.813, 
German has been less optimized; %only 0.687, which may imply that German has been less optimized during language evolution; 
this finding is in line with \citet{gildea2010grammars}, where %\citet{gildea2010grammars} 
the authors observed that DDM has a much weaker impact on German than on English. %, with both exhibiting DDM though. 
}

\fix{
On the other hand, \textbf{diacrhonic} investigation of dependency distance has received an increasing interest in the past few years (e.g., \citet{zhang2023investigation,zhu2022investigating,liu2022dependency}). \citet{tily2010role} may be the first relevant work.\footnote{Although \citet{lei2020dependency,zhang2023investigation} claim that \citet{lei2020dependency} is the first diachronic approach for DDM, we argue that this is not true.} 
%to explore the diachronic trend of dependency distance.
He found that the total dependency distance of English sentences decreased %over time 
from 900 to 1500 (from Old English to Early Modern English). As the corpora only contain constituency annotations, 
he %had to 
automatically converted the annotations into dependency annotations for analysis. 
Subsequently, \citet{gulordava-merlo-2015-diachronic} compared Latin / ancient Greek from different time periods using manually annotated dependency treebanks, finding that languages from the earlier periods exhibit lower DDM levels against the optimum
than those from the later periods. 
More recent studies leveraged dependency parsers to automatically parse the sentences extracted from diachronic corpora, and then based their observations on the parsing results \citep{lei2020dependency,juzek2020exploring,liu2022dependency,zhu2022investigating,zhang2023investigation,krielke2023optimizing}. An important benefit of such studies is that they do not require the expensive dependency annotations%for dependency
; therefore, arbitrary corpora beyond treebanks can serve as the research resource. \citet{lei2020dependency,liu2022dependency} investigated the diachronic trend of dependency distance based on the State of the Union Addresses corpus \citep{}, which contains the political speeches of 43 U.S. presidents from 1790 to 2017. They showed that the \mdd{} and its normalized metric (\ndd{}) \citep{lei2020normalized} of American English sentences are decreasing over time. While \citet{lei2020dependency} observed a consistent downward trend across different sentence length groups% including that of less than 10 words
, contradicting the anti-\ddm{} principle for short sentences \citep{ferrer2021anti}, \citet{liu2022dependency} additionally divided 
%sentence group of less than 10 words 
the sentences of $\leq$ 10 words (the shortest sentence group in \citet{lei2020dependency}) into two subgroups: sentences of 0-4 and 5-10 words, finding that the anti-\ddm{} phenomenon does exist for the 0-4 group. 
%\citet{juzek2020exploring} 
\citet{zhu2022investigating,zhang2023investigation} compared the diachronic trend of \mdd{} and/or \ndd{} across varying text genres, based on the COHA \citep{} corpus; it contains the texts in American English for the past 100-200 years in 4 domains: News, Magazine, Fiction, Non-fiction. Generally, their findings are inconsistent. E.g., \citet{zhu2022investigating} found a downtrend of \mdd{} only for the Fiction genre %, while 
and an upward trend
%was observed 
for the News and Magazine genres. In contrast, \citet{zhang2023investigation} %examined the texts in News and Magazine genres,  
observed a general decrease in \mdd{} and \ndd{} for the Magazine genre over time. Nevertheless, both of their results imply that the diachronic trend of \mdd{} is inconsistent across various text genres. 
\citet{juzek2020exploring} explored the diachronic shifts in syntactic patterns for scientific English, leveraging the Royal Society Corpus \citep{}, which comprises the scientific publications from 1665 to 1996. They also observed a decrease in \mdd{} over time.
As the follow-up work, \citet{krielke2023optimizing} %more 
comprehensively investigated %the 
language optimization for scientific English and German from 1650 to 1900, in comparison to that for general languages. She found that while the \mdd{} for scientific languages decreased over time, \mdd{} for general languages does not show a chronological decrease during the same period. %She also argued that 
%confirm the downtrend of \mdd{} in scientific
}

\par{
\fix{\citet{lei2020dependency,liu2022dependency}
divided sentences into different groups according to their length. Specifically, they grouped the sentences into those having 1-10 (0-4, 5-10), 11-20, 21-30, and 31+ words. \citet{zhang2023investigation,juzek2020exploring,krielke2023optimizing} compared sentences of the same length.  
}

\fix{\citet{Yih2022HowSA}: the effect of annotation schemes on the dependency distance}


%Previous studies on diachronic syntactic language change focus on the changes in dependency distance. The principle of dependency distance minimization (DDM) %as an important indicator of language complexity, 
%has been researched a lot. On the one hand, many studies have shown that the mean dependency distance (or its variant) of a real sentence is shorter than that of the random baselines (e.g., the sentence with random word orders), from a synchronic perspective. 
%\todo{add semantic change as well}

%\citet{futrell2015large} investigated DDM in 37 languages. They provided the first large-scale evidence of DDM, which suggests that DDM may be a universal property of all languages. They used the parsed corpora of 37 different languages to perform the tests 
%and showed that the dependency distance of real sentences is shorter than chance. This indicates that languages indeed have undergone optimization.   

%\citet{gildea2010grammars} observed that DDM has a much weaker impact on German than on English. They reordered the sentences so that it has the minimal possible dependency length and then compared it to that of the original sentences, in order to explore at what level the language has been optimized. They found that the dependency length of both English and German are significantly less than random; however, the effect of DDM is substantially smaller in German compared to English.

%We extract the dependencies from natural language text and reorder the words in such a way as to minimize dependency length. Comparing the original text with these optimal linearizations (and also with random linearizations) reveals the degree to which natural language minimizes dependency length. Tests on English data show that English shows a strong effect of DLM, with dependency length much closer to optimal than to random; the optimal English grammar also has many specific features in common with English. In German, too, dependency length is significantly less than random, but the effect is much weaker than in English.

%\citet{ferrer2022optimality} analyzed the optimality for 93 languages from 19 linguistic families. They defined a new metric that can measure the optimality of a certain language and the resulting cognitive pressure based on the dependency distance. Their results suggest that 50\% of the languages are optimized to a level of at least 70\%. Compared to English, which obtains an optimality score of 0.813, German achieves only 0.687, which may imply that German has been less optimized during language evolution. This finding is in line with \citet{gildea2010grammars}.


%\citet{futrell2015large,ferrer2022optimality} compared DDM across 37/97 languages from varying linguistic families and showed that the degrees of DDM vary for different languages; however, their comparison was limited to a synchronic scope as the used treebanks only contain the data for a small time span. 

%\citet{lei2020dependency} is the first work that studies DDM from a diachronic perspective. They observed a consistent decline in dependency distance in the State of the Union Addresses corpus, spanning 227 years. Additionally, they noted a prominent tendency toward Dependency Distance Minimization (DDM) in shorter sentences, those typically containing ten words or fewer.

\iffalse
\citet{juzek2020exploring}
explored diachronic shifts in syntactic usage patterns within Scientific English, focusing on the period from around 1700 to 1900 using the Royal Society Corpus (RSC) containing publications from the Royal Society of London. The hypothesis posited that evolving syntactic preferences over time lead to greater dependency locality, improving communication efficiency in expert-to-expert exchanges. With the RSC corpus, the research identified a trend towards shorter dependency structures, reflecting a shift towards enhanced communicative efficiency over the years.

%\citet{liu2022dependency}

\citet{liu2022dependency} studied the effects of sentence lengths and dependency types on DDM, using the corpus in the political domain that covers 227 years. Noting that \citet{ferrer2021anti} and \citet{lei2020dependency} have inconsistent conclusions about the DDM in short sentences, they conducted the analysis with a more fine-grained grouping of sentence lengths. Specifically, they further divided the sentences of length less than 10 words into groups 0-4 and 5-10. They demonstrated that the mean dependency distance of sentences having less than 5 words is increasing, while that of the sentences having 5-10 words is decreasing over time. Their findings support the anti-DDM hypothesis proposed by \citet{ferrer2021anti}. Additionally, they also showed that longer sentences contain more dependency relations, whose dependency distance decreases over time; this may explain why the longer sentences are more influenced by DDM than the short ones. 

\citet{zhu2022investigating} investigated the diachronic trend of dependency distance for texts in different genres. Specifically, they examined the language change for texts in four genres: fiction, news, magazine, and non-fiction, using %They used 
the COHA corpus, which spans from 1900-2009. %To do so, 
They performed the Mann-Kendall trend test \citep{mann1945nonparametric} to detect the trend 
in the dependency distance. Their results suggest that 
%They showed that 
the downtrend of dependency distance is inconsistent across various genres. The dependency distance is decreasing only in fiction texts over time, while it shows an uptrend for the other three genres. It is worth noting that they are the only approach that compared sentences of exactly the same length, while the others grouped the sentences with different bin sizes, which may be the reason why the downtrend is weak in their experiment. In Section \ref{sec:analysis}, we discuss the effect of the bin size used for sentence grouping on the distribution of sentence length in the resulting dataset. Generally, a bin size of 5 already has a large impact, as there is a clear tendency for shorter sentences to appear more frequently in the later decades compared to the earlier decades; thus, the sentences in the same length group will be shorter for the later time periods and vice versa.
\fi
%They  

%\citet{zhang2023investigation} also studied the diachronic trend of dependency distance
%Lei and Wen., 2020; Liu et al., 2022; Juzek et al., 2020; Zhu et al., 2022; Zhang and Zhou, 2023 analyzed dependency distance based on diachronic corpora covering large time spans, but all explored corpora are for English. Moreover, all of the mentioned diachronic investigations leveraged the Stanford CoreNLP parser, which was not specifically trained and evaluated on historical data; therefore, it may have led to biased conclusions, as a consequence of incorrect parsing.

 

%language change and dependency parsing.

%\subsection{Language Change}

%In recent years, researchers explored the evolution of language change, from both 

%Many studies have shown that human languages are being optimized towards lower complexity and higher efficiency in terms of communication \citep{gibson2019efficiency,ferrer2022optimality,degaetano2022toward}
%[Gibson et al., 2019; Ferrer-i-Cancho 2022; Degaetano-Ortlieb, and Teich 2019]. 
%Among others, syntactic dependency distance, i.e., the linear distance between syntactically dependent words, is often perceived as the indicator of language processing difficulty and working memory load of humans \citep{temperley2007minimization,liu2008dependency,zhu2022investigating,juzek2020exploring}.
%[Temperley, 2007; Liu, 2008; Liu et al., 2017; Zhu et al. 2022; Juzek et al. 2020]. 
%The corresponding optimization principle is well-established,  i.e., dependency distance minimization (DDM), which refers to the tendency/preference of syntactically related words being placed closer to each other.


%A large array of works have confirmed the existence of DDm in natural languages (e.g., \citet{temperley2007minimization,futrell2015large,juzek2020exploring,zhang-etal-2020-efficient}).
%[Temperley, 2007; Furtrell et al., 2015; Juzek et al., 2020; Zhang and Zhou, 2023]. 
%On the one hand, studies suggest that the mean dependency distance (or its variant) of a real sentence is shorter than that of the random baselines (e.g., the sentence with random word orders) and this may be a universal property of most natural languages [Gildea and Temperly, 2010; Furtrell et al., 2015; Ferrer-i-Cancho et al., 2022]. On the other hand, there is also evidence of DDm found in the diachronic investigations of (English) language change, i.e., the dependency distance generally decreases over time [Lei and Wen., 2020; Liu et al., 2022; Juzek et al., 2020; Zhang and Zhou, 2023; Zhu et al., 2022]. However, it is still unanswered whether the trend of diachronic DDm is generalizable to other languages. Furtrell et al., 2015; Ferrer-i-Cancho et al., 2022 compared DDm across 37/97 languages from varying linguistic families and showed that the degrees of DDm indeed vary for different languages; however, their comparison was limited to a synchronic scope as the used treebanks only contain the data for a small time span. Gildea and Temperly, 2010 observed that DDm has a much weaker impact on German than on English, also from a synchronic perspective. Lei and Wen., 2020; Liu et al., 2022; Juzek et al., 2020; Zhu et al., 2022; Zhang and Zhou, 2023 analyzed dependency distance based on diachronic corpora covering large time spans, but all explored corpora are for English. Moreover, all of the mentioned diachronic investigations leveraged the Stanford CoreNLP parser, which was not specifically trained and evaluated on historical data; therefore, it may have led to biased conclusions, as a consequence of incorrect parsing. Furthermore, DDm has been identified as the origination of other manifestations of syntactic structure optimizations, such as the scarcity of crossing dependencies (Gómez-Rodríguez and Ferrer-i-Cancho, 2017; Ferrer-i-Cancho and Carlos Gómez-Rodríguez, 2021), and can even predict other principles of language optimization beyond syntax like the minimization of word lengths (Ferrer-i-Cancho and Carlos Gómez-Rodríguez, 2021); these highlight the importance of studying DDm for understanding language change. 





==> structure_unused/3_data.tex <==
\section{Data Preparation}
\label{sec:data}
\paragraph{\textbf{Corpora}}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\textwidth]{figs/preprocessing.png}
    \caption{4-step preprocessing pipeline for sentence extraction from the corpora.}
    \label{fig:preprocessing}
\end{figure}
\todo{redo the figure with tikz; maybe put in intro}
In this work, we use corpora consisting of political debates and speeches in both languages to ensure a fair comparison. For \textbf{English}, we select the \textbf{\texttt{Hansard}} corpus, which comprises the official reports of UK parliament debates.
To compile the data for the time period 1803—2004, we extract XML files from the Hansard archive\footnote{\url{https://www.hansard-archive.parliament.uk/}}, retaining every section labeled as ``debate''. 
%In this work, we consider corpora containing political debates/speeches for both languages, for a fairer comparison. We choose the \textbf{\texttt{Hansard}} corpus for \textbf{English}, which contains the official reports of UK parliament debates. For the data for the time period 1803---2004, we crawl XML files from Hansard archive\footnote{\url{https://www.hansard-archive.parliament.uk/}} and retreat every section marked with ``debate'' valid.
Data from 2005 to April 2021 is obtained from a Zenodo repository.\footnote{\url{https://evanodell.com/projects/datasets/hansard-data/} (v3.1.0)} 
As for \textbf{German}, we utilize the \textbf{\texttt{DeuParl}} corpus published by \citet{FairGer}; it contains plenary protocols from both the Reichstag (the former German parliament) and the Bundestag (the current German parliament), covering the period from 1803 to 2022.
%spanning the period from 1803 to 2022.

\paragraph{\textbf{Preprocessing}}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=.5\linewidth]{figs/hansard_data.png}
    \hspace{1cm}
    \includegraphics[width=.15\linewidth]{figs/hansard_data2.png}
    \caption{Screenshot of data snippets in the Hansard corpus.}
    \label{fig:data_hansard}
    
\end{figure}


\begin{figure}[!ht]
    \centering
    \includegraphics[width=.5\linewidth]{figs/deuparl_data1.png}
    \includegraphics[width=.45\linewidth]{figs/deuparl_data2.png}
    \caption{Screenshot of data snippets in the DeuParl corpus.}
    \label{fig:data_deuparl}
    
\end{figure}

To extract sentences from the corpora, we employ a 4-step preprocessing approach, outlined in Figure \ref{fig:preprocessing}. Initially, we conduct preprocessing at the paragraph level, with the aim of providing cleaner inputs for the sentence tokenizer. For example, as Figure \ref{fig:data_hansard} (left) shows,
in the original data of Hansard, the page numbers are often not excluded from the sentence due to OCR errors, which occupy an individual line (``[238''). In DeuParl, the text is often split into lines by periods, no matter whether they serve as the ending punctuation. As shown in Figure \ref{fig:data_deuparl}, ``z.B.'' is accidentally split into two lines (left figure); a similar case exists for ``27. März'' in the right figure. With paragraph-level preprocessing, we delete the line break and the page numbers (for example) before applying the sentence tokenizer to the text.

In the case of DeuParl, which is in plain text format, we divide each file into paragraphs of 50 lines, in order to ensure not to exceed the maximum input length of the sentence tokenizer. For \texttt{Hansard}, the paragraphs are naturally organized within the XML files. Subsequently, we utilize Spacy \citep{spacy2} %with state-of-the-art (SOTA) models 
to segment the paragraphs into sentences. The next step involves 
postprocessing on the segmented paragraphs, primarily focused on correcting errors stemming from the sentence tokenizer. For instance, ``hon.'' often appears in the Hansard corpus as the abbreviation of ``honorable'', which is sometimes perceived as the end of a sentence by the sentence tokenizer. Furthermore, we find inconsistent usage of semicolons as sentence-ending punctuation. For example, in the UD treebanks, semicolons are occasionally permitted as the concluding punctuation of sentences; at other times, multiple individual sentences connected by semicolons are treated as one sentence. However, the sentence tokenizer tends to split the sentences by semicolons.
%In this work, we d
With simple postprocessing, we manage to correct such errors of segmentation.
Finally, we apply a filtering process to exclude texts that may not qualify as complete and standalone sentences;
%To extract sentences from the corpora, we do 4-step preprocessing, as illustrated in Figure \ref{fig:preprocessing}. %\todo{add pipeline figure}
%First, we do preprocessing on paragraph-level, aiming to provide more clean inputs to the sentence tokenizer. As \texttt{DeuParl} is in plain text format, we divide each file into paragraphs of 50 lines, avoiding exceeding the maximal input length of the sentence tokenizer; for \texttt{Hansard}, the paragraphs are naturally the paragraphs in the XML files. Next, we use Spacy \citet{} with the SOTA models\footnote{For English, we use xxx, while for German, we use xxx.} to split the paragraphs into sentences. Then, sentence-level preprocessing is performed to correct some errors from the sentence tokenizer. Finally, we filter out those texts that may not be complete and standalone sentences 
this is achieved through the following simple and intuitive rules: 
\begin{itemize}
    \item Sentences must start with a capitalized character.
    \item Sentences must end with a period, or a question mark, or an exclamation mark.
    \item Sentences must contain a verb based on the part-of-speeching tags.
    \item The number of (double) quotation marks must be even.
    \item The number of %the 
    left brackets must be equal to that of %the 
    right brackets.
\end{itemize} 

It is possible that such preprocessing/filtering biases the results later discussed to some extent, as some sentences may have been ignored through it; however, %as shown in Figure \ref{}, \todo{add incomplete sentence segment example here.}
directly applying sentence segmentation to the original data leads to incomplete sentence segments or data from other parts, e.g., a budget table, as Figure \ref{fig:data_hansard} (right) shows, %\todo{add example?}
which can 
result in larger biases for the mismatch with the 
definition 
%the input 
of the dependency parsing task, i.e., parsing the syntactic structure of a sentence, and consequently affect the measures calculated on a sentence level.
%input of most dependency parsers, i.e., sentences. %, and with the way of mean dependency distance calculation, i.e., 

%and the way of , i.e., they parse the text on sentence-level, and with how the dependency distance is calculated,  

\subsection{Validation \& Correction}
To validate the feasibility of our preprocessing pipeline
and study the influence of data noise on measures such as dependency distance (discussed in Section \ref{sec:analysis}), for each corpus, 
%we apply it to 5 randomly sampled paragraphs from each decade, totaling $\sim$150-800 sentences per decade, then manually review 10 random outputs for each decade, and correct them if any issues are identified. The data from 2020s is merged into 2010s, as there is only data for 2 years. %, which is few compared to the others.
We apply it to five randomly sampled paragraphs from each decade, resulting in approximately 150-800 sentences per decade. We then manually review ten randomly selected outputs for each decade and make corrections if any issues are identified. Additionally, the data from the 2020s is merged into the 2010s, given that only partial data is available for the former.

\paragraph{\textbf{Annotation}}
We first check the \textbf{German} sentences from \texttt{DeuParl}. Two annotators with an NLP background, one male faculty member who is a German native, and one female PhD student who speaks German fluently, check the outputs. In this phase, we do not have annotation guidelines; the annotators are asked to freely make comments on each text from their intuition and make corrections if they identify any issues in the text.\footnote{The annotation is done with Google spreadsheet.} 
%, freely document the issues found in the text, and correct them if any are identified; in this phase, we do not have annotation guidelines.
Subsequently, by inspecting the comments and comparing them to the original PDF files,\footnote{\url{}} \todo{find the website}
we standardize and format the annotation scheme. As Figure \ref{fig:annotation} shows, %\todo{add screenshot of the annotation}
the formatted annotation has 5 columns: 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/annotation2.png}
    \caption{Screenshot of the formatted annotation.}
    \label{fig:annotation}
\end{figure}

%\begin{enumerate}[(1)]
\begin{itemize}
    \item \textbf{\large (1) is\_sent}: A \textbf{binary} annotation (`TRUE'/`FALSE') for sentence identification, i.e., whether the text is a sentence (minor issues in the sentence, such as space or spelling errors, are allowed).
    \item \textbf{\large (2) has\_issues}: A \textbf{binary} annotation about the existence of any issues (only if (1) is `TRUE').
    \item \textbf{\large (3) issues}: A sequence of labels for the \textbf{category of the issues} identified, e.g., spelling errors. 
    (only if (1) and (2) are `TRUE'). 
    %the issues are classified into x categories: \emph{xxx}, \emph{xxx}. 
    \item \textbf{\large (4) origin\_of\_issues}: A sequence of labels for the \textbf{origin of the issues}. For example, if some spelling errors are a consequence of OCR errors, then the ``origin'' of them should be ``OCR''.
    %including xxx, xxx, and xxx; 
    The labels here are aligned in
    a one-to-one manner with those in (3) (only if (1) and (2) are `TRUE').
    \item \textbf{\large (5) correction}: The \textbf{corrected sentence} (only if (1) and (2) are `TRUE').
    %\item (1) \textbf{\large correction}: The corrected sentence.
%\end{enumerate}
\end{itemize}

\begin{table}[!ht]
\begin{tabularx}{\textwidth} { >{\hsize=.2\hsize}X | >{\hsize=.5\hsize}X | >{\hsize=.3\hsize}X }
\toprule
Category              & Example                                                                                                                                                                                                                                                & Correction                           \\ \midrule
Spelling              & Das ist die Mehrheit; die Diskussion ist {\color[HTML]{FE0000} geschloffen}.                                                                                                                                                                                                  & {[}...{]} geschlossen.               \\\midrule
Space                 & Der EVG-Vertrag spreche von der „westlichen Verteidigung", und im Protokoll der NATO-Staaten sei vom Zusammenschluß der {\color[HTML]{FE0000}w e s t europäischen} Länder die Rede.                                                                                          & {[}...{]} westeuropäischen {[}...{]} \\\midrule
Missing Material      & Ich bin der Meinung — und viele an uns herangekommene Klagen lassen auch darauf schließen {\color[HTML]{FE0000}—} , dass die Auffassung des Reichssparkommissars, dass das Personal der Deutschen Reichspost voll ausgelastet, aber nicht überlastet sei, nicht richtig ist. & add ``—''                            \\\midrule
Extra Material        & %Aber die oft vertretenen Vorschläge meiner Fraktion haben während des Krieges bei allen {\color[HTML]{FE0000}(0)} übrigen Parteien eine Beachtung nicht gefunden.   
[...] daß durch den Bund zweierlei Recht für die Norddeutschen geschaffen werden soll, {\color[HTML]{FE0000}(Sehr richtig!)} daß gewissermaßen zweierlei Klassen von Norddeutschen geschaffen werden sollen, {\color[HTML]{FE0000}(Sehr gut!)} eine Selekta, die vermöge ihrer Gesittung [...]

& delete ``(Sehr gut!)'' and  ``(Sehr richtig!)''                       \\\midrule
\makecell{Punctuation \\\& \\Symbol}
 & Ich bitte, daß diejenigen Herren, welche für den Fall der Annahme des {\color[HTML]{FE0000}Z} 33b in demselben die Worte „oder an Druck m anderen öffentlichen Orten" aufrecht erhalten wollen, sich von ihren Plätzen erheben.                                              & %replace ``Z'' with ``§'' 
 [...] § 33b [...]\\ \bottomrule
\end{tabularx}
\caption{Categories of issues; each is shown with an example and the corresponding correction. The parts having a certain issue or missing in the sentences are in \textcolor{red}{red}.}
\label{tab:issue_example}
\end{table}



%The categories of the issues are listed in Table \ref{tab:issue_example}. 
We classify the issues into 5 categories: \emph{Spelling}, \emph{Space}, \emph{Missing Material}, \emph{Extra Material} and \emph{Punctuation \& Symbol}, as shown in Table \ref{tab:issue_example}. Additionally, we split the origins of issues into 4 categories: (1) \emph{Historic}, which indicates the issues are due to the differences in historical and modern language. For example, ``daß'' is a spelling issue with the \emph{historic} origin. (2) \emph{OCR}, which indicates the issue is an OCR error. For example, the spelling issue in Table \ref{tab:issue_example} results from the OCR error. (3) \emph{Genre}, which represents the issues that exist due to the characteristics of the text genre. In the text of the political debate genre, the language changes between written and spoken language frequently, and also, there exist interjections within a sentence, as shown in the fourth row of Table \ref{tab:issue_example} (extra material). (4) \emph{Preprocessing}, which denotes that the issues stem from our preprocessing pipeline. For details regarding those categories, 
we refer to Figure \ref{fig:annotation} in the appendix, which demonstrates 
our annotation guidelines for Hansard following the refined annotation scheme.


%we examine the origins of the issues by checking the original PDF files.  

%and the categories of the issue origins are presented in Table \ref{}.  \todo{add one table displaying the issue categories.}


Next, two annotators annotate the \textbf{English} text from \texttt{Hansard}, following the annotation scheme defined above. 
%The annotations guidelines are shown in \pdf
As the original PDF files of Hansard are inaccessible, we can not identify the origins of the issues; thus, this annotation is omitted for Hansard.
Among the annotators, one is a male faculty member, while the other is a female Master's student, both with an NLP background.


%\includepdf[]{figs/annotation_guidelines.pdf}
%\includepdf[pages=1-2,scale=.8,picturecommand*={\put (\LenToUnit{.05\paperwidth},20) {};}]{figs/annotation_guidelines.pdf}
\iffalse
\begin{figure*}[ht]
	\centering
	\includegraphics[width=\linewidth]{figs/annotation_guidelines.pdf}
	\caption{fig zonder benen}
	\label{fig:blabla}
\end{figure*}


\begin{figure}[!ht]
    \centering
    \includepdf[pages=1-2,scale=.8,picturecommand*={\put (\LenToUnit{.05\paperwidth},20) {};}]{figs/annotation_guidelines.pdf}
    \caption{Annotation Guidelines for the formatted annotation scheme.}
    \label{fig:anno_gruideline}
\end{figure}
\fi

%\paragraph{\textbf{Agreement}}
%Based on the formatted annotation, we then calculate the inter-agreement between the two annotators. 
To check the \textbf{agreement} among annotators,
40 German sentences are jointly annotated, 20 for the sentence identification task and 20 for the issue identification/correction task. As for English, 30 sentences are commonly annotated for all annotation subtasks.
For each binary annotation task, we calculate Cohen's Kappa for inter-agreement, whereas for the correction task,  
%For (1) and (2), we directly calculate the Kappa agreement, while for (3) and (4), we first convert the annotations into one-hot vectors, representing the appearance of the labels, as Figure \ref{} shows. \todo{add example for one-hot vector.}
%As for (5), 
we compute the edit distance between sentences. Let $s$ be the original sentence, and $s'_{a}$ and $s'_{b}$ be the sentences corrected by annotators A and B respectively. We calculate the edit distance (i) between $s$ and $s'_{a}$ ($ED(s,s'_{a})$), (ii) between $s$ and $s'_{b}$ ($ED(s,s'_{b})$), and (iii)  between $s'_{a}$ and $s'_{b}$ ($ED(s'_{a},s'_{b})$). %We argue that 
If the corrections are similar to each other, (i) and (ii) should be close while (iii) should be small. %xxxx 
\todo{why?}
Overall, the annotators obtained a decent level of agreement, with $\sim$ 0.7 on binary tasks and the edit distances of (i) = 3.88, (ii) = 3.96, and (iii) = 0.54 for the correction.

%between (i) the original sentence and the corrected one by annotator A, (ii) the original sentence and the corrected one by annotator B, and (iii) the corrected sentence by A and that by B.
Furthermore, as the formatting of German annotations was not done by the annotators themselves, we also checked whether they agreed with the formatted annotations made by us. To do so, we let them both check the formatted annotations for the same 30 sentences. 
The annotators only disagreed on two sentences, because the OCR spelling errors have been omitted. 
%\todo{then?}

%Generally, the annotators obtain decent agreements on all annotation tasks (xxx-xxx Kappa)....
%a bit low in issues, because of omitting the historical spelling? also for agreement on reformat??

%Then, we adopt the formatted annotation scheme to \textbf{English} sentences.
%Two annotators annotated 10 common ones, obtaining xxx-xxx kappa for tasks (1)-(4), and xxx ED...
%low (1) -> discussion until agreement -> 

\iffalse
deuaprl:
4/40 are different; is_sent kappa:  0.688715953307393
4/40 are different; has_issues kappa:  0.7808219178082192
24: 0.5833333333333334 - 4.041666666666667 - 4.125


hansasrd:
30
4/30 are different, is_sent kappa:  -0.05263157894736836
1/26 are different, has_errors kappa:  0.7796610169491526
2: 0.0 - 2.0 - 2.0


ALL:
70 - is_sent kappa:  0.5364238410596026
66 - has_issues kappa:  0.84593837535014
26: 0.5384615384615384 - 3.8846153846153846 - 3.9615384615384617

\fi

\begin{figure}[!ht]
    \centering
    %\flushleft
    \begin{subfigure}[t]{0.5\textwidth}
        \includegraphics[width=\linewidth]{figs/deuparl_is_sent_160.png}
        \caption{Deuparl}
        %\label{fig:enter-label}
    \end{subfigure}%
    \begin{subfigure}[t]{0.5\textwidth}
        \includegraphics[width=\linewidth]{figs/hansard_is_sent_220.png}
        \caption{Hansard}
        %\label{fig:enter-label}
    \end{subfigure}%
    \caption{Distribution of the texts identified as perfect sentences (without any issues), sentences with issues, and non-sentences over time.}
    \label{fig:is_sent}
\end{figure}

\begin{figure}[!ht]
    %\centering
    \flushleft
    \begin{subfigure}[t]{0.37\textwidth}
        \includegraphics[width=\linewidth]{figs/deuparl_issues_154.png}
        \caption{\textbf{Deuparl} - issues}
        \label{fig:de_issue}
    \end{subfigure}%
    \hspace{-.3cm}
    \begin{subfigure}[t]{0.25\textwidth}
        \includegraphics[width=\linewidth]{figs/deuparl_origins_73.png}
        \caption{\textbf{Deuparl} - origins}
        \label{fig:de_origin}
    \end{subfigure}%
    \hspace{.2cm}
    \begin{subfigure}[t]{0.37\textwidth}
        \includegraphics[width=\linewidth]{figs/hansard_issues_218.png}
        \caption{\textbf{Hansard} - issues}
        \label{fig:en_issue}
    \end{subfigure}%
    \caption{(a)/(c): Percentage of perfect sentences and sentences with a specific issue to all texts identified as sentences. (b): Percentage of sentences with issues from a specific origin to all sentences containing issues.}
    \label{fig:sent_quality}
    \vspace{-.3cm}
\end{figure}


\paragraph{\textbf{Results}}

We show the distribution of the texts identified as perfect sentences (without any issues), sentences with issues, and non-sentences in Figure \ref{fig:is_sent}. 
We observe that: (1) German data has more issues compared to English. For the older time periods, e.g., the first 3 decades in each corpus, 60-70\% German sentences are found to contain issues, while there are only 20-30\% English sentences that are found to be problematic. (2) Only a small portion of sentences were identified as non-sentence. Specifically, 6 out of 160 texts ($\sim$3.75\%) from Deuparl and 2 out of 220 texts ($\sim$0.1\%) from Hansard are found not to be sentences. 
(3) The proportion of problematic sentences is decreasing over time; for both languages, all sentences after 2000 are flawless.

Next, we present the percentages of the sentences having a specific issue in Figure \ref{fig:de_issue} and Figure \ref{fig:en_issue}. The category \emph{Symbol} is merged into \emph{Punct} here. 
Note that one sentence can have multiple issues, so the sum of the percentages does not need to equal 100\%. In English data, 90\% of the sentences are perfect---only 1\%-2\% of the sentences have \emph{Spelling}, \emph{Space}, or \emph{Punct} issues. In contrast, only half of the German sentences are issue-free, with over 40\% of the sentences having \emph{Spelling} issues and 1\%-5\% of the sentences containing other issues. Furthermore, we find that \emph{Historic} origin issues dominate in the problematic German sentences---
over 55\% of those contain at least one \emph{Historic} origin issue, followed by \emph{OCR} origin---$\sim$30\% of the flawed sentences have issues raised from OCR errors. 

In summary, our annotations suggest that English data from \texttt{Hansard} is substantially less problematic than the German data from \texttt{Deuparl}. Notably, the most prevalent issues %existing 
in the German data, %are 
%the 
namely historical spelling and OCR spelling error, %which, 
by contrast, 
rarely appear in the English data. %This raises our doubts 
This leads us to question whether the \texttt{Hansard} Corpus has already undergone preprocessing like spelling normalization. %etc
Through contact with the UK Parliament enquiry services,\footnote{\url{https://www.parliament.uk/site-information/contact-us/}} 
we received feedback indicating that the data has not been preprocessed regarding spelling normalization. As for OCR errors, a statement on their website\footnote{\url{https://hansard.parliament.uk/about}} explicitly mentions that OCR errors are curated once identified. As a consequence, 
%those facts imply that 
we conclude that English has undergone smaller changes in terms of spelling in the past 200 years, compared to German.
%xxxxx \todo{add a statement that }


\iffalse
\begin{figure}[!ht]
    \centering
    %\flushleft
    \begin{subfigure}[t]{0.49\textwidth}
        \includegraphics[width=\linewidth]{figs/deuparl_is_sent_160.png}
        \caption{Distribution of labels for the sentence identification task over time.}
        %\label{fig:enter-label}
    \end{subfigure}%
    \begin{subfigure}[t]{0.28\textwidth}
        \includegraphics[width=\linewidth]{figs/deuparl_issues_154.png}
        \caption{Percentage of perfect sentences and sentences with a specific issue to all texts identified as sentences.}
        %\label{fig:enter-label}
    \end{subfigure}%
    %\hspace{.2cm}
    \flushright
    \begin{subfigure}[t]{0.18\textwidth}
        \includegraphics[width=\linewidth]{figs/deuparl_origins_73.png}
        \caption{Percentage of sentences with issues from a specific origin to all sentences containing issues.}
        %\label{fig:enter-label}
    \end{subfigure}%
    \caption{Deuparl}
    \label{fig:deuparl_quality}
    \vspace{-.3cm}
\end{figure}
\fi

%\todo{add figures for issue presentation; add examples of different types of issues.}


%\subsection{Correction}
%Apart from the sentences collected in the validation phase, one annotator continues to correct more German sentences, resulting in xxx English and xxx German corrected sentences in total, together with the previous ones. 


%\paragraph{\textbf{ChatGPT vs. Humans}}

%\todo{add classification report -> high precision on positive category 
%; edit distance -> correction  german special case } 

==> structure_unused/4_parser.tex <==
\section{Dependency Parsers}\label{sec:parser}

Unlike previous approaches, which often solely relied on a single parser, typically the Stanford CoreNLP Parser \citep{manning-etal-2014-stanford}, we will base our observations on 
%a range of dependency 
various parsers with the two most popular design choices: transition-based and graph-based.
Transition-based parsers sequentially predict the arc step by step based on the current state,
while graph-based parsers globally optimize the dependency tree, aiming to find the highest-scored one. The parsers used in this work include: (1) \textbf{transition-based}: CoreNLP \citep{manning-etal-2014-stanford}, StackPointer \citep{ma-etal-2018-stack}; (2) \textbf{graph-based}: Biaffine \citep{dozat2016deep}, Stanza \citep{qi-etal-2020-stanza}, TowerParse \citep{glavas-vulic-2021-climbing} and CRF2O \citep{zhang-etal-2020-efficient}. %Note that CoreNLP and CRF2O are incapable of predicting crossing edges.

\iffalse
\paragraph{\textbf{Transition-based Parsers}}\todo{add explanation of each parser type}
\begin{itemize}
    \item CoreNLP \citep{manning-etal-2014-stanford}:
    %We use it with the out-of-box setting except for disabling sentence splitting; 
    \textbf{unable to predict non-projective relations.}
    \item StackPointer \citep{ma-etal-2018-stack} 
\end{itemize}
\paragraph{\textbf{Graph-based Parser}}
\begin{itemize}
    \item Deep Biaffine \citep{dozat2016deep}
    \item Stanza \citep{qi-etal-2020-stanza}: a deep Biaffine parser with additional features that predict the linearization order of the words and the linear distance between the words.
    \item TowerParse \citep{glavas-vulic-2021-climbing}: %de: HDT en: EWT
    \item CRF2O \citep{zhang-etal-2020-efficient}: an extension to the Deep Biaffine parser with the second-order TreeCRF; \textbf{unable to predict non-projective relations.} %(only for English) 
\end{itemize}
%\iffalse
\paragraph{\textbf{Span-based}}
\begin{itemize}
    \item MRC
\end{itemize}
\fi
%\todo{add the citation of parsers; maybe add one parser for sequence generation-based ones?}
We train model checkpoints for StackPointer, Biaffine, and CRF2O on the concatenated train set of the treebanks in UD2.12, separately for each language.\footnote{We use the implementation of Biaffine and CRF2O from \url{https://github.com/yzhangcs/parser}, StackPointer from \url{https://github.com/XuezheMax/NeuroNLP2}.} 
The authors of TowerParse released the checkpoints trained on individual treebanks in UD2.5; %however, 
as they did not provide the training script, we directly take the models trained on the largest treebank for each language, i.e., EWT for English and HDT for German.\footnote{\url{https://github.com/codogogo/towerparse}}
For CoreNLP and Stanza,
we use them with the out-of-the-box setting.\footnote{We use Stanza of version 1.5.1 and CoreNLP via the client API bundled in Stanza.}
%, while we train model checkpoints  
Note that the default models in Stanza 1.5.1 were also trained using UD2.12, %, there is
however,
the default German model is only trained on the GSD treebank, and the default English model is trained on the combination of 5 out of 7 train sets in the treebanks.

Except for Stackpointer, which does not have a built-in tokenizer, and CoreNLP, which has its own tokenizer, the other parsers implement the tokenizer from Stanza by default. Thus, for ease of use,
%to have a better insight into the discrepancy in the parsing approaches, 
we implement the Stanza tokenizer for every parser consistently, disabling sentence segmentation, as we will apply them to the curated sentences from our target corpora, for which further sentence splitting is unexpected.

\subsection{Evaluation}
\par To explore the reliability of the parsers used, we evaluate them on (1) existing \textbf{UD treebanks}, (2) the treebanks built upon the two target corpora of this work (denoted as ``\textbf{Target Treebanks}''), and (3) adversarially attacked treebanks concerning two of the most severe issues identified in Section \ref{sec:data}. 

\paragraph{\textbf{Metrics}} 
We calculate the \textbf{Unlabeled Attachment Score (UAS)} and \textbf{Labeled Attachment Score (LAS)} for the parser performance. UAS and LAS are originally defined as the percentage of tokens with correctly predicted heads and head+relations respectively; in this scenario, the input of the parser is sentences pre-tokenized by humans. On the other hand, \citet{zeman-EtAl:2018:K18-2} test the parsers' performance in a real-world scenario, i.e., parsing the raw text without any gold standard (e.g., sentence segmentation, tokenization, part-of-speech tags, etc.). %and re-define the two metrics as follows:
%\todo{add formula}
The metrics are then re-defined as the the harmonic mean (F1) of precision
P and recall R, where P is the percentage of the correct \fix{head (+relation)} to the number \fix{of} predicted tokens, while \fix{R} is the percentage of the correct \fix{head (+relation)} to the number of tokens in the gold standard.


As we will use the parsers on %plain texts containing curated 
%not tokenized 
sentences without tokenization, we argue that \emph{the re-defined metrics on raw texts are more indicative in our case}.  
For all evaluations, we adopt the evaluation script\footnote{\url{https://universaldependencies.org/conll18/evaluation.html}} from the CoNLL18 dependency shared task \citep{zeman-EtAl:2018:K18-2} with a slight modification, allowing for comparing the subtypes
%\zr{new term what subtypes?} 
of relations as well. 

\subsubsection{Evaluation on UD Treebanks} 
To ensure the correctness of the training, implementation, and usage of the %used 
parsers, we first evaluate the parsers on the test sets of the existing UD treebanks, for which we choose Universal Dependencies (UD) v2.12,\footnote{We exclude the treebank ``GumReddit'' for English, as there are many nonsensical annotations.} 
and compare the results to %those reported in 
\citet{zeman-EtAl:2018:K18-2}. Although our evaluation setup, parsers, and the version of the UD treebanks are 
%slightly 
different from theirs,
%there differ from those we use in this work, 
comparable (or better) results are expected since the discrepancy in UD versions is small\footnote{Most changes are about fixing a tiny portion of incorrect annotations, e.g., see change logs on \url{https://github.com/UniversalDependencies/UD_English-PUD/blob/master/README.md} and \url{https://github.com/UniversalDependencies/UD_German-GSD/blob/master/README.md}.}. Most of the tested parsers are published later than the shared task where the parsers do not need to split the text into sentences by themselves.

\begin{figure}[!ht]
    \centering
    \begin{subfigure}[t]{0.48\linewidth}
        \includegraphics[width=\linewidth]{figs/en_pud.png}
        \caption{EN-PUD}
        \label{fig:enter-label}
    \end{subfigure}%
    \begin{subfigure}[t]{0.5\linewidth}
        \includegraphics[width=\linewidth]{figs/de_gsd.png}
        \caption{DE-GSD}
        \label{fig:enter-label}
    \end{subfigure}%
    \caption{Barplot of LAS of the parsers in our evaluation in comparison to the \textcolor{red}{average} and the \textcolor{blue}{best} LAS over various parsers on the English PUD and German GSD test sets reported in Table 15 of \citet{zeman-EtAl:2018:K18-2}. }
    \label{fig:conll}
    \vspace{-.3cm}
\end{figure}

%We merged the test sets of multiple treebanks for a specific language into a whole one. 
%The statistics of the merged treebanks are presented in Table \ref{}. 
%\todo{add a table to show how many word pairs are in the treebanks, as well as the original corpora and relevant information like the time periods.} 

\paragraph{\textbf{Results}}
We first compare our evaluation results on one random treebank to that reported in \citet{zeman-EtAl:2018:K18-2}  for each language. As Figure \ref{fig:conll} displays, the great majority of the parsers obtain higher LAS than the average LAS over parsers in \citet{zeman-EtAl:2018:K18-2}, except for CRF2O on German, whose LAS is slightly lower than the average. Stanza, Towerparse, and Biaffine consistently outperform the best systems across different languages. Thus, we confirm the legitimacy of the used parsers. 
%\zr{would be interesting to know parser performance by design choices.} 
\todo{feel not enough}
%the legitimacy of the parsers has been confirmed.

\begin{table}[!ht]
\centering
\begin{subtable}[t]{0.7\linewidth}
%\centering
\resizebox{\linewidth}{!}{% 
\begin{tabular}{@{}lcc|cc@{}}
\toprule
\multicolumn{1}{l}{} & \multicolumn{2}{c|}{UAS}                 & \multicolumn{2}{c}{LAS}                  \\
                     & UD                & TARGET               & UD                & TARGET               \\ \midrule
CoreNLP*              & 78.6±5.5          & 82.9 (+4.3)          & 73.4±6.5          & 78.7 (+5.3)          \\
Stanza*               & \underline{88.2±6.2}    & 88.0 (-0.2)          & \underline{84.9±8.0}    & 85.0 (+0.1)    \\
TowerParse*           & 87.1±4.5          & \textbf{92.8 (+5.7)} & 82.8±5.9          & \textbf{90.3 (+7.5)} \\
StackPointer         & 85.7±5.2          & 84.2 (-1.5)          & 81.3±6.2          & 80.2 (-1.1)          \\
CRF2O                & 87.2±4.6          & 86.6 (-0.6)          & 83.5±5.4          & 82.8 (-0.7)          \\
Biaffine             & \textbf{91.6±2.6} & \underline{90.1 (-1.5)}    & \textbf{88.5±3.3} & \underline{87.2 (-1.3)}          \\ \bottomrule
\end{tabular}%
}%
\caption{English}
\label{tab:parser_de}
\end{subtable}%

\begin{subtable}[t]{0.7\linewidth}
%\centering
\resizebox{\linewidth}{!}{% 
\begin{tabular}{@{}lcc|cc@{}}
\toprule
             & \multicolumn{2}{c|}{UAS}                 & \multicolumn{2}{c}{LAS}                  \\
             & UD                & TARGET               & UD                & TARGET               \\ \midrule
CoreNLP*      & 74.0±2.9          & 74.4 (+0.4)          & 67.3±2.9          & 69.6 (+2.3)          \\
Stanza*       & 84.3±4.1          & 87.6 (+3.3)          & 78.8±4.4          & 82.0 (+3.2)          \\
TowerParse*   & \underline{86.2±2.0}    & \underline{89.7 (+3.5)}    & \underline{80.3±1.3}    & \underline{84.5 (+4.2)}    \\
StackPointer & 83.6±1.3          & 86.9 (+3.3)          & 78.2±1.6          & 80.8 (+2.6)          \\
CRF2O        & 78.5±1.5          & 81.9 (+3.4)          & 70.2±2.4          & 72.9 (+2.7)          \\
Biaffine     & \textbf{87.0±2.5} & \textbf{90.8 (+3.8)} & \textbf{81.7±1.8} & \textbf{84.5 (+2.8)} \\ \bottomrule
\end{tabular}%
}%
\caption{German}
\label{tab:parser_de}
\end{subtable}%
\caption{UAS and LAS on \texttt{\textbf{UD}} and \texttt{\textbf{Target}} treebanks. We show the macro average and the standard deviation of the metrics over the UD treebanks. The best performance in each criterion is bold and the second best one is underlined. We mark the parsers trained on mismatched data (with respect to UD versions or treebanks) with $^{*}$.}
\label{tab:parser_eval}

\end{table}



Next, we show the macro average and the standard deviation of the UAS
%(a) 
and LAS 
%(b) 
over the UD treebanks in Figure \ref{tab:parser_eval} (column ``\textbf{UD}''). %For English, we 
Biaffine consistently outperforms the others across different languages in terms of both UAS (en: 92\% vs. 79\%-88\%;
%for English and 
de: 87\% vs. 79\%-86\% for German) and LAS (en: 89\% vs. 73\%-85\%; 
%for English and 
de: 82\% vs. 70\%-80\%). 
%for German). 
Furthermore, it also exhibits the strongest robustness across various treebanks, as demonstrated by the smallest average standard deviation ($\sim$2.55 percentage points (pp)) over different metrics and languages. It is noteworthy that CoreNLP, the parser leveraged by all other related approaches, is the worst in our evaluation, according to all criteria.

Stanza %with the out-of-the-box setting 
trained on slightly mismatched data outperforms the other fine-tuned ones on average for English. Nevertheless, it is the least robust one according to its high standard deviations (6.2 pp vs. <5.5 pp in UAS; 8.0 pp vs. <6.5 pp in LAS). Interestingly, Towerparse, without any treebank- and/or version-specific fine-tuning, performs similarly to Biaffine on German treebanks,  only $\sim$1 pp lower UAS/LAS. However, we observe that it tends to predict multiple roots for one sentence and produce cycles in the dependency tree graphs. In our evaluation, it generates 440 multi-root predictions and 1,498 cycles, %for xxx 
%\zr{maybe one example?} 
%sentences in the treebanks, \todo{add size of test set}
while the others rarely make such errors (only Stackpointer predicts multiple roots 28 times). Besides, it also has to skip 28 sentences due to the limitation of its implementation.\footnote{See authors' explanation about skipping sentences in footnote 7 of \citet{glavas-vulic-2021-climbing}.}
CRF2O performs on par with the second-tier parsers on English data but is the worst one on German data. The reason may be that it is not capable of parsing non-projective relations, which 
%obviously 
%exist much more 
occur more frequently in German compared to English. %\zr{any reference?}%\citep{}. 
With its built-in evaluation function, which skips the non-projective sentences in the gold standard ($\sim$3k out of $\sim$23k sentences), the UAS and LAS raise from <80\% to >90\% on German treebanks.  

%\todo{maybe add the results for pre-tokenized sentences}
%For English, except for CoreNLP, the others 

%In the evaluation of \citet{zeman-EtAl:2018:K18-2}, dependency parsers obtain 70\%-75\% LAS on the easiest English and German treebanks on average, which indicates a slightly lower performance than the parsers evaluated here (70\%-89\%). 
%whereas thethe parsers evaluated here obtain 70\%-80\% LAS  




\iffalse
\begin{table*}[!ht]
%\flushleft
\begin{subtable}[t]{0.48\linewidth}
%\centering
\resizebox{\linewidth}{!}{% 
\begin{tabular}[t]{@{}l|cc|cc@{}}
\toprule
             & \multicolumn{2}{c|}{\underline{\textbf{EN}}}      & \multicolumn{2}{c}{\underline{\textbf{DE}}}      \\
parser       & UD                & Target & UD                & Target \\ \midrule
corenlp      & 78.6±5.5          & 82.9     &  \_         &  \_    \\
stanza       & 88.2±6.2          & 88.0     & 84.3±4.1          & 87.6     \\
towerparse   & 87.1±4.5          & \textbf{92.8}     & 86.2±2.0          & \textbf{89.7}     \\ \midrule
stackpointer & 85.7±5.2          & 84.2     & 83.6±1.3          & 86.9     \\
crf2o        & 87.2±4.6          & 86.6     & 78.5±1.5          & 81.9     \\
biaffine     & \textbf{91.6±2.6} & 90.1     & \textbf{87.0±2.5} & \textbf{90.8}     \\ \bottomrule
\end{tabular}%
}%
\caption{UAS}
\label{tab:uas}
\end{subtable}%
%\centering
%\flushright
\hspace{.2cm}
\begin{subtable}[t]{0.48\linewidth}
%\centering
\resizebox{\linewidth}{!}{% 
\begin{tabular}[t]{@{}l|cc|cc@{}}
\toprule
             & \multicolumn{2}{c|}{\underline{\textbf{EN}}}      & \multicolumn{2}{c}{\underline{\textbf{DE}}}            \\
parser       & UD                & Target      & UD                & Target      \\ \midrule
corenlp      & 73.4±6.5          & 78.7          & \_           & \_           \\
stanza       & 84.9±8.0          & 85.0          & 78.8±4.4          & 82.0          \\
towerparse   & 82.8±5.9          & \textbf{90.3} & 80.3±1.3          & 84.5          \\ \midrule
stackpointer & 81.3±6.2          & 80.2          & 78.2±1.6          & 80.8          \\
crf2o        & 83.5±5.4          & 82.8          & 70.2±2.4          & 72.9          \\
biaffine     & \textbf{88.5±3.3} & 87.2          & \textbf{81.7±1.8} & \textbf{84.5} \\ \bottomrule
\end{tabular}%
}%
\caption{LAS}
\label{tab:las}
\end{subtable}%
\caption{UAS and LAS on \texttt{\textbf{UD}} and \texttt{\textbf{Target}} treebanks. We show the macro average and the standard deviation of the metrics over the UD treebanks. The best performance is underlined. We mark the parsers trained on mismatched data (with respect to UD versions or treebanks) with $^{*}$.}
\label{tab:parser_eval}
\vspace{-.4cm}
\end{table*}
\fi




\subsubsection{Evaluation on Target Treebanks}
We leverage the dependency annotation in UD format collected in the DoTT project, \todo{add citation}
which includes 111 sentences from Hansard and 163 from DeuParl. 

\iffalse
As previous related works only explore parsers' performance on diachronic data for English, we collect more annotations for German sentences, which allows for a fair evaluation of parsers over time. 

To do so, we first check the dates of the sentences from DoTT by searching in our data or online.\footnote{We found a mismatch between the years reported in their paper and those identified by us. As we are unclear how the authors sampled the sentences, we decided to use the dates identified by ourselves.} 
Additionally, we collect annotations for xxx Deuparl sentences to balance the annotated data across both sentence lengths and time periods. The annotation was done by one annotator, who is a Master's student majoring in German language. We use Google Spreadsheet as the annotation tool, as the screenshot shown in Figure \ref{}.\todo{add annotation screenshot}
Before starting to annotate new sentences, the annotator annotated 12 sentences (xxx tokens) sampled from DoTT, obtaining xxx UAS and xxx LAS. He was then asked to check the discrepancy in the annotations and correct the ones that he argued were his own errors, leading to an increasing agreement (xxx UAS and xxx LAS). Subsequently, on another 12 sentences (xxx tokens) sampled from DoTT, the agreement achieves a decent level: xxx UAS and xxx LAS. \todo{maybe report kappa.}
We summarize the statistics of the final \texttt{Target Treebanks} in Table \ref{}.\todo{add table to present the annotated data: time periods, sentence lengths, how many with known dates?}
\fi

\paragraph{\textbf{Results}}
We show the evaluation results on the Target treebank in Table \ref{tab:parser_eval} (column ``\textbf{Target}''). The values in the brackets indicate the absolute difference in metrics between the Target treebank and the UD treebanks. We observe that the Target treebank mostly does not negatively 
%\zr{odd verb "comparable but mildly worse?"}
affect the parsers' performance. All parsers exhibit improved performance on the \textbf{German} Target treebank compared to the UD treebank, with an increase ranging from 0.4 to 4.2 pp. For \textbf{English}, the maximal performance drop is observed with StackPointer and Biaffine (1.1-1.5 pp), while CoreNLP and TowerParse achieve better results, with an increase ranging from 4.3 to 7.5 pp. Stanza and CRF2O display only minor fluctuations (<1 pp). Hence, our results suggest that these parsers are able to parse the sentences in the target domain.


\iffalse
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[!ht]
\centering
\resizebox{.6\textwidth}{!}{%
\begin{tabular}{@{}l|cc|cc@{}}
\toprule
             & \multicolumn{2}{c|}{\underline{en}}      & \multicolumn{2}{c}{\underline{de}}       \\
parser       & UD                & historic & UD                & historic \\ \midrule
corenlp      & 78.6±5.5          & 82.9     & 22.4±2.6          & 19.6     \\
stanza       & 88.2±6.2          & 88.0     & 84.3±4.1          & 87.6     \\
towerparse   & 87.1±4.5          & \textbf{92.8}     & 86.2±2.0          & \texbf{89.7}     \\ \midrule
stackpointer & 85.7±5.2          & 84.2     & 83.6±1.3          & 86.9     \\
crf2o        & 87.2±4.6          & 86.6     & 78.5±1.5          & 81.9     \\
biaffine     & \textbf{91.6±2.6} & 90.1     & \textbf{87.0±2.5} & \textbf{90.8}     \\ \bottomrule
\end{tabular}
}
\caption{UAS}
\label{tab:uas}
\end{table}

\begin{table}[!ht]
\centering
\resizebox{.6\textwidth}{!}{%
\begin{tabular}{@{}l|cc|cc@{}}
\toprule
             & \multicolumn{2}{l|}{en}           & \multicolumn{2}{l}{de}            \\
parser       & UD                & historic      & UD                & historic      \\ \midrule
corenlp      & 73.4±6.5          & 78.7          & 4.7±1.0           & 2.2           \\
stanza       & 84.9±8.0          & 85.0          & 78.8±4.4          & 82.0          \\
towerparse   & 82.8±5.9          & \textbf{90.3} & 80.3±1.3          & 84.5          \\ \midrule
stackpointer & 81.3±6.2          & 80.2          & 78.2±1.6          & 80.8          \\
crf2o        & 83.5±5.4          & 82.8          & 70.2±2.4          & 72.9          \\
biaffine     & \textbf{88.5±3.3} & 87.2          & \textbf{81.7±1.8} & \textbf{84.5} \\ \bottomrule
\end{tabular}
}
\caption{LAS}
\label{tab:las}
\end{table}
\fi


\begin{figure}[!ht]
\vspace{-.2cm}
    \centering
    \begin{subfigure}[t]{0.5\linewidth}
        \includegraphics[width=\linewidth]{figs/adv_attack_his.png}
        \caption{Historical Spelling Attack}
        \label{fig:attack_his}
    \end{subfigure}%
    \hspace{1cm}
    \begin{subfigure}[t]{0.4\linewidth}
        \includegraphics[width=\linewidth]{figs/adv_attack_ocr_legend.png}
    \end{subfigure}%
    
    \begin{subfigure}[t]{\linewidth}
        \includegraphics[width=\linewidth]{figs/adv_attack_ocr.png}
        \caption{OCR Spelling Attack}
        \label{fig:attack_ocr}
    \end{subfigure}%
    \caption{Absolute difference in UAS and LAS between the sentences before and after the attack.}
    \label{fig:attack}
    \vspace{-.3cm}
\end{figure}


\subsubsection{Evaluation on Adversarial Treebanks}
Our adversarial attacks concern the two most prevalent issues in German data identified in Section \ref{sec:data}, i.e., historical spelling and OCR-raised spelling errors. We perturb the merged German test set to create the adversarial treebanks. 
To perform the historical spelling attack, we chose 23 candidate words from our previous annotations and replaced them with their historical spellings in the test set. This resulted in 1,971 sentences that were affected by the attack. 
%\zr{maybe more detail on the 23 candidate words, why choose them? }
%(xxx tokens). 
For (2), we randomly replace 10\%, 30\%, or 50\% of the characters in 1 or 2 tokens within a sentence with random characters, resulting in 6 attacking levels; we produce 2000 sentences per attack level. 
%, resulting in xxx perturbed sentences (xxx tokens).

\paragraph{\textbf{Results}}

We illustrate the absolute difference in metrics between the sentences before and after attacking in Figure \ref{fig:attack}. Both types of attacks consistently have a greater influence on LAS compared to UAS. This can be explained by that LAS is more sensitive to perturbations because it considers both attachment and labeling accuracy, whereas UAS only considers attachment accuracy. Even if the attachment remains correct, changes to the words themselves (such as spelling or character replacement) can result in incorrect labels. As depicted in Figure \ref{fig:attack_his}, \textbf{historical spelling} has a slight negative impact on the parsers' performance, with a difference of less than 0.07 in LAS and that of up to around 0.05 in UAS. Among the parsers, Biaffine is the most stable one, followed by TowerParse; CoreNLP exhibits the lowest robustness. 

We present the results for \textbf{OCR spelling attack} in Figure \ref{fig:attack_ocr}. OCR spelling errors have a slightly larger impact, degrading the parsers' performance up to around 0.12 in LAS and 0.09 in UAS, when 50\% characters of 2 tokens within a sentence are perturbed. Again, Biaffine is the most robust one against OCR attack, followed by CRF2O and TowerParse, which demonstrate similar sensitivity to Biaffine when the attack level is high. At the highest attack level, CoreNLP, StackPointer, and Stanza show similar sensitivity. However, at low attack levels, StackPointer and Stanza demonstrate better robustness compared to CoreNLP. In real-world cases, OCR spelling errors often involve only one character within a sentence. For example, in the sentence ``...
%Diesen freien Menschen, die dort Tag und Nacht an ihrer Arbeit sitzen,
wollen \emph{Tie} nun das letzte nehmen.'' (from our annotation in Section \ref{sec:data}), the only OCR error is in ``\emph{Tie}'', which should be corrected to ``\emph{Sie}''. Hence, Stanza and StackPointer are still superior to CoreNLP in real-world scenarios.

%as shown in Figure \ref{fig:attack_ocr}. Nevertheless, 

\subsection{Summary}
%\paragraph{\textbf{Summary}}
Among the explored parsers, Biaffine shows the best performance in standard evaluations as well as the highest robustness under adversarial conditions. CoreNLP and CRF2O are often the worst ones in our evaluation. Besides,
%CoreNLP and CRF2O 
they are unable to predict crossing edges, 
which we deem as an important indicator of language change. 
%Besides, they often the worst 
%Further, 
Non-projective sentences seem to substantially degrade CRF2O's performance; thus, we exclude it from further experiments. CoreNLP is retained, however, for comparison purposes. Therefore, \emph{we will use five parsers to perform the large-scale analysis in Section \ref{sec:analysis}; they are: CoreNLP, StackPointer, Biaffine, TowerParse, and Stanza.}

==> structure_unused/5_analysis.tex <==
\section{Analysis}\label{sec:analysis}
\subsection{Datasets}

\begin{figure}[!ht]
    \centering
    \begin{subfigure}[t]{0.5\linewidth}
        \includegraphics[width=\linewidth]{figs/en_len_dis_random.png}
        \caption{Hansard}
        \label{fig:len_dis_en}
    \end{subfigure}%
    \begin{subfigure}[t]{0.5\linewidth}
        \includegraphics[width=\linewidth]{figs/de_len_dis_random.png}
        \caption{Deuparl}
        \label{fig:len_dis_de}
    \end{subfigure}%
    \caption{The distribution of sentence length with the bin size of 3 for the randomly sampled sentences having at most 100 tokens (which occupy 99\% of the random dataset). We grouped the time periods by every 2 decades, except for year 2023, which was merged into the 2000 decade group.}
    \label{fig:len_dis}
    \vspace{-.3cm}
\end{figure}

%show the distribution, average of the sentence lengths and the time periods.

We apply the preprocessing pipeline introduced in Section \ref{sec:data} to
get up to 200k sentences for each decade and language, and then use the five parsers to parse the sentences. From those sentences, we generate 2 datasets for observation: 
%\begin{itemize}
\paragraph{\textbf{\texttt{Random}}}
    %\item \textbf{\texttt{Random}}: 
    We randomly sample 2k sentences from each decade. The distribution of sentence length is illustrated in Figure \ref{fig:len_dis}. We see a clear trend that there are \fix{more} shorter sentences in the later decades and vice versa. %The main 
%\paragraph{\textbf{\texttt{ChatRandom}}}
    %\item \textbf{\texttt{ChatRandom}}: 
    %We use ChatGPT to filter out non-sentence texts and also let ChatGPT correct the sentences for German; 2k random sentences curated by ChatGPT are retained per decade for both languages.
\paragraph{\textbf{\texttt{Balance}}}
    %\item \textbf{\texttt{Balance}}: 
    Since sentence length plays a great role in measures like dependency distance \citep{lei2020dependency,zhu2022investigating,zhang2023investigation}, we carefully create a balanced dataset across sentence lengths. The sentence length is calculated as 
    %We treat 
    the number of tokens in sentences tokenized by Stanza.
    %as the sentence length.
    To ensure sufficient sentences for each length group and time period, we group every two decades together (with 2020 as an exception, which is grouped into the 2000 decade group), and select 450 sentences for each of the %with 
    anchor lengths [5, 10, 15, 20, 30, 40, 50, 60, 70] %for each 
    per decade group. The balanced dataset has $\sim$1905 sentences per decade for German 
    (450 $\times$ 9 length groups $\times$ 8 decade groups $\div$ 17 decades $\approx$ 1905) and $\sim$1937 sentences per decade for English.
    %$\div$ 2 decades $\approx$ 2k sentences per decade). 
    In our initial experiment, we grouped sentences in bins of size 5; for example, sentences of lengths 20-24 were placed in the group of anchor length 20. Nevertheless, such a grouping strategy leads to unbalanced data because the earlier decade groups tended to have \fix{more} longer sentences of lengths close to the upper bound and vice versa%of length close to the %anchor length
    %upperbound
    ---the mean sentence length in the resulting dataset is consequently decreasing over time and 
    that of decade group 2000 is 5 
    %times smaller 
    \fix{tokens} less than that of group 1860 for German, for example.\todo{need to check the exact number}
    Thus, we restrict the bin size to 3 for length grouping; the final dataset has differences of less than 0.1 in mean sentence length across decade groups.%, and no downtrend 
    %for both English and German.  
%\end{itemize}
%(1) We randomly sample 2k sentences from each decade, denoted as \textit{Random}. (2) We use ChatGPT to filter out non-sentence texts and also let ChatGPT correct the sentences for German; 2k random sentences curated by ChatGPT are retained per decade for both languages (denoted as \textit{ChatRandom}). (3) Since %many works have shown that 
%sentence length plays a great role in measures like dependency distance \citep{lei2020dependency,zhu2022investigating,zhang2023investigation}, we create a fully balanced dataset across sentence lengths. To ensure sufficient sentences for each length group and time period, we group every two decades together and select sentences with anchor lengths [5, 10, 15, 20, 30, 40, 50, 60, 70] for each decade group. In our initial experiment, we group sentences in bins of size 5; for example, sentences with lengths of 20-24 are placed in one length group. However, such grouping strategy still led to unbalanced data because 

\iffalse
and group them in bins of size 5.  However, such grouping 


In our initial experiment, we gro

To get sufficient numbers of sentences 

The anchor sentence lengths consider 
For this, we need to carefully select the length groups. 
In our initial experiment, we grouped the sentences with a bin size of 5, 

We first select sentences of length [5, 10, 15, 20, 30, 40, 50, 60, 70] for each decade. Observing that 

To get sufficient amount of sentences of each sente
\fi
%the 5 parsers to parse up to 200,000 sentences 



\subsection{Measures}

\begin{figure}[!ht]
    \centering
    \begin{subfigure}[t]{0.7\linewidth}
        \includegraphics[width=\linewidth]{figs/measure_example.png}
        \caption{Linear order}
        \label{fig:tree_example_a}
    \end{subfigure}%
    \begin{subfigure}[t]{0.3\linewidth}
        \includegraphics[width=\linewidth]{figs/example_tree.png}
        \caption{Tree graph}
        \label{fig:tree_example_b}
    \end{subfigure}%
    \caption{Dependency relations of sentence ``Das hat alles sehr gut geklappt!'' (taken from the German GSD treebank of UD), illustrated in (a) linear order and (b) tree graph. Numbers in the brackets in (b) denote the positions of the tokens in the sentence and the numbers beside the edges (in blue) refer to the dependency distance between the dependent-head token pairs.}
    \label{fig:tree_example}

\end{figure}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[!h]
\begin{tabular}{@{}lr@{}}
\toprule
MDD           & 2.6  \\
NDD & 0.84 \\
Tree Height                              & 3    \\
\#Crossing            & 1    \\
\#Leaves                    & 3    \\
Tree Degree           & 3    \\
Longest Path Distance        & 13   \\
Left Children Ratio              & 0.67  \\
Depth Variance                      & 0.47 \\
Depth mean                         & 1.17 \\
Degree Variance                     & 1.14 \\
Degree Mean                         & 0.83 \\
Topological Order Distance     & 4    \\
Random Tree Distance         & 4    \\ \bottomrule
\end{tabular}
\caption{Measures for the dependency relations in Figure \ref{fig:tree_example}.}
\label{tab:tree_example}
\end{table}

Unlike most other approaches that only focus on the linear dependency distance (e.g., \citet{lei2020dependency,liu2022dependency,zhu2022investigating,zhang2023investigation}), we examine a large array of measures based on the properties of the tree graphs. We visualize the dependency relations in both linear order and tree graph for an example sentence in Figure \ref{fig:tree_example} and list the corresponding measures in Table \ref{tab:tree_example}.
The 15 measures considered in this work include:
\begin{itemize}
    \item \textbf{Mean Dependency Distance (MDD)} \& \textbf{Normalized Mean Dependency Distance (NDD)}. %\paragraph{}
    Following \citet{lei2020dependency,zhang2023investigation}, %\todo{citaiton missing}
    we compute the MDD and its variation, NDD, proposed by \citet{lei2020normalized}, which normalizes the MDD according to the root position and the sentence length. MDD is the average distance between depend-head pairs within a sentence. 
    Punctuations are excluded from the calculation. 

    \item \textbf{Root Distance}. The position of the root token in a sentence. E.g., the root distance for the sentence in Figure \ref{fig:tree_example} is 6 (root: ``geklappt''). 
    
    \item \textbf{Number of Crossings (\#Crossing)}. Crossings or non-projectivity refers to edges crossing over each other when the dependency relations are illustrated in the predefined linear order. We calculate the number of crossing edges, excluding those attached to punctuations. E.g., 
    as shown in Figure \ref{fig:tree_example_a}, the edge between ``Das'' and ``alles'' is crossing over that between ``geklappt'' and ``hat'', while the other edges are not crossing; thus, $\#Crossing = 1$. 

    %\item \textbf{Arity/Tree Degree}. 
    \item \textbf{Tree Height}. The height of the dependency tree. It is 3 for the given example in Figure \ref{fig:tree_example_b}.

    \item \textbf{Depth Variance \& Depth Mean}. The variance and mean of node depths within the tree. 
    In Figure \ref{fig:tree_example_b}, for instance, 'geklappt' has a depth of 0, while 'sehr' has a depth of 2. Punctuations are excluded. For the tree in Figure \ref{fig:tree_example_b}, the depth mean is 1.17 and the depth variance is 0.47.
    
    \item \textbf{Arity/Tree Degree}. The maximal degree of a node in a tree, where \emph{degree of a node} is defined as the number of its children. In Figure \ref{fig:tree_example_b}, node ``geklappt'' has the maximal number of children (3), excluding the exclamation mark, so the degree of the tree is 3.
    
    \item \textbf{Degree Variance \& Degree Mean}. The variance and mean of node degrees within the tree. Punctuations are excluded. For the tree in Figure \ref{fig:tree_example_b}, the degree mean is 0.83 and the degree variance is 1.14. 
    
    \item \textbf{Number of leaves (\#Leaves)}. The number of leaves of the tree. Punctuations are excluded. The tree in Figure \ref{fig:tree_example_b} has three leaves: ``alles'', ``hat'', and ``sehr''. 
    
    \item \textbf{Left Children Ratio}. We calculate the ratio of the left children of a node to all its children, then average it over the nodes having at least one child in a tree. For example, in the phrase "the methods used", ``used'' is a right child of ``methods'', while in ``the used methods'', which expresses exactly the same meaning, ``used'' is a left child of ``methods''. We also exclude punctuation here.\todo{maybe change to head-final percentage ``The effects of sentence length on dependency distance,
dependency direction and the implications–Based on a
parallel English–Chinese dependency treebank''; ``Dependency direction as a means of word-order typology:
A method based on dependency treebanks''}
    
    \item \textbf{Longest Path Distance}. The maximal sum of dependency distance along the path from the pseudo root to a leaf. In Figure \ref{fig:tree_example_b}, the longest path is observed with ``root''---``Das''---``alles'', so the sum distance is 13.
    
    \item \textbf{Topological Order Distance}. 
    %Topological sort returns a sequence of nodes where each node appears before the nodes it points to.
    By topological sorting, we ensure that in the sorted array, each dependent node appears before its head. The root will then be placed at the end of the sorted array. The sentence in Figure \ref{fig:tree_example_a} after topological sorting will be ``alles Das hat sehr gut ! geklappt'', and then, we compute the Levenshtein edit distance \citep{Levenshtein1965BinaryCC} %\todo{add citation}
    between the original %sentence 
    and the sorted sentence on the token level. %instead of character-level. 
    %, so the root token will be at the end of the sorted sequence.
    
    \item \textbf{Random Tree Distance}. We randomly generate a tree with the same number of nodes, and then compute the tree edit distance between the original and the random trees using the algorithm of \citet{zhang1989}.
    
\end{itemize}



\subsection{Trend Test}

%bdlf;FJN;LSFHSKJDFHD
Following \citet{zhu2022investigating}, %\todo{add citation}
we perform the Mann Kendall (MK) trend test \citep{mann1945nonparametric} to indicate the diachronic change of the concerned measures. Mann Kendall trend test is widely used to detect trends in the time series. Additionally, as some measures are obviously highly correlated to the sentence length, such as the tree height and root distance, we perform another modified version of MK, namely the partial Mann Kendall (PMK) test \citep{libiseller2002performance}, which reduces the influence of other independent variables on the response variable by considering the conditional distribution of the MK statistics. In our case, we perform the PMK trend test for the measures in the presence of the sentence length. For both trend tests, we use the implementation from \citet{Hussain2019pyMannKendall}.






%\paragraph{\textbf{}}

\subsection{Results}


\noindent\textbf{RQ1: %\emph{%Do the issues identified in the sentences impact on the measures?
Are those measures sensitive to the data noise?}\\%}\\

\noindent To assess the sensitivity of the measures to the noise in the sentences, we compute Spearman's $\rho$ correlations between the measures on the original and human corrected sentences (collected in Section \ref{sec:data}). Higher correlations indicate less impact and vice versa---if the noise does not disrupt measure rankings, it is considered on an acceptable level. 

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[!ht]
\resizebox{.85\linewidth}{!}{% 
\begin{tabular}{@{}ccccccc@{}}
\toprule
\multicolumn{1}{l|}{Measures}                                & stanza & corenlp & stackpointer & biaffine & \multicolumn{1}{c|}{towerparse}                 & AVG   \\ \midrule
\multicolumn{1}{l|}{MDD}                  & 0.976  & 0.905   & 0.823        & 0.966    & \multicolumn{1}{c|}{0.888} & 0.912 \\
\multicolumn{1}{l|}{NDD}                  & 0.995  & 0.892   & 0.862        & 0.985    & \multicolumn{1}{c|}{0.960} & 0.939 \\
\multicolumn{1}{l|}{Tree Height}               & 0.983  & 0.915   & 0.862        & 0.986    & \multicolumn{1}{c|}{0.820} & 0.913 \\
\multicolumn{1}{l|}{Left Children Ratio}   & 0.975  & 0.954   & 0.959        & 0.972    & \multicolumn{1}{c|}{0.909} & \textbf{0.954} \\
\multicolumn{1}{l|}{Tree Degree}               & 0.968  & 0.916   & 0.870        & 0.973    & \multicolumn{1}{c|}{0.815} & 0.908 \\
\multicolumn{1}{l|}{\#Leaves}          & 0.998  & 0.999   & 0.908        & 0.997    & \multicolumn{1}{c|}{0.832} & 0.947 \\
\multicolumn{1}{l|}{Degree Variance}          & 0.966  & 0.935   & 0.923        & 0.976    & \multicolumn{1}{c|}{0.834} & 0.927 \\
\multicolumn{1}{l|}{Degree Mean}         & 0.998  & 0.988   & 0.902        & 0.998    & \multicolumn{1}{c|}{0.832} & 0.944 \\
\multicolumn{1}{l|}{Depth Variance}           & 0.982  & 0.910   & 0.861        & 0.976    & \multicolumn{1}{c|}{0.827} & 0.911 \\
\multicolumn{1}{l|}{Depth Mean}          & 0.987  & 0.918   & 0.874        & 0.980    & \multicolumn{1}{c|}{0.818} & 0.915 \\
\multicolumn{1}{l|}{Topological Order Distance} & 0.989  & 0.967   & 0.891        & 0.990    & \multicolumn{1}{c|}{0.841} & 0.936 \\
\multicolumn{1}{l|}{\#Crossing}        & 0.942  & -       & 0.815        & 0.938    & \multicolumn{1}{c|}{0.782} & \underline{0.869} \\
\multicolumn{1}{l|}{Longest Path Distance}        & 0.995  & 0.935   & 0.874        & 0.994    & \multicolumn{1}{c|}{0.884} & 0.936 \\
\multicolumn{1}{l|}{Root Distance}       & 0.999  & 0.870   & 0.873        & 0.965    & \multicolumn{1}{c|}{0.976} & 0.937 \\
\multicolumn{1}{l|}{Random Tree Distance} & 0.991  & 0.991   & 0.894        & 0.986    & \multicolumn{1}{c|}{0.830} & 0.938 \\ \midrule
\multicolumn{1}{l|}{AVG}                  & \textbf{0.983}  & 0.935   & 0.879        & 0.979    & \multicolumn{1}{c|}{\underline{0.857}} & 0.926 \\ \bottomrule
\end{tabular}%
}%
\caption{Spearman's $\rho$ between the measures on the original sentences and that on the human-corrected sentences (collected in Section \ref{sec:data}). The ``AVG'' values in the rows refer to the average correlation over different parsers for a specific measure; those in the columns denote the average correlation over different measures for a specific parser. 
%We bold the lowest average correlations.
We bold the highest and underline the lowest average correlations.}
\label{tab:corr_measure}
\end{table}

%\todo{maybe additionally show the correlation between trend tests results on random and chatrandom dataset.}
%show the correlation of the measures on the original and corrected sentences.


Overall, as
Figure \ref{tab:corr_measure} illustrates,
%a strong overall correlation (0.926) between 
the measures on the original and corrected sentences strongly correlate with each other, shown with an overall %average 
correlation of 0.926. This overall correlation is computed by first averaging over parsers for each measure and then averaging over all measures. The lowest average correlation per measure is observed with \#crossing, 0.869, which, however, still implies a strong correlation. The least sensitive measure is the left-children ratio, shown with an average correlation of 0.954 over parsers. Among the parsers, Stanza is least sensitive (0.983), followed by Biaffine (0.979), whereas TowerParse and StackPointer are the most sensitive ones (0.857 and 0.879 respectively). As a consequence, we conclude that \emph{\textbf{those measures are consistently insensitive to the data noise across different parsers}}.


\vspace{1cm}\noindent\textbf{RQ2: \emph{Do the dependency parsers agree with each other?}}\\

\noindent Next, we investigate the impact of using different parsers on the diachronic trend analysis. To do so, we calculate the Cohen's Kappa agreement between the results of the trend tests based on different parsers. The trend tests have three outputs: ``no trend'', ``decreasing'' and ``increasing'', which can be seen as the labels of a three-way classification task. We use all trend test outputs on the \texttt{Random} and \texttt{Balance} datasets, resulting in 330 test cases for each %parser and 
language (2 trend tests $\times$ 15 measures $\times$ (1 trend on \texttt{Random} + 1 overall trend on \texttt{Balance} + 9 trends on \texttt{Balance} for different sentence length groups) = 330). We then calculate the agreement on the 330 trends between the parsers. 

\begin{figure}[!ht]
    \centering
    \begin{subfigure}[t]{0.51\linewidth}
        \includegraphics[width=\linewidth]{figs/hansard_parser_corr_all.png}
        \caption{Hansard}
        \label{fig:parser_cor_en}
    \end{subfigure}%\hspace{-.8cm}
    \begin{subfigure}[t]{0.51\linewidth}
        \includegraphics[width=\linewidth]{figs/deuparl_parser_corr_all.png}
        \caption{Deuparl}
        \label{fig:parser_cor_de}
    \end{subfigure}%
    \caption{Cohen's Kappa between the results of the original and partial Mann Kendall trend test based on the dependency relations predicted by different parsers. Deeper colors denote higher agreement and vice versa. We show the average agreement for each parser in the last row.}
    \label{fig:parser_cor}
    \vspace{-.3cm}
\end{figure}

We show the agreement matrix in Figure \ref{fig:parser_cor}. Most parsers demonstrate a moderate to high agreement with others (0.6-0.8). On \textbf{English} data, as illustrated in Figure \ref{fig:parser_cor_en}, the highest agreement of 0.85 is observed between Stanza and StackPointer, succeeded by Stanza and Biaffine (0.78); Stanza obtains the highest average agreement with others (0.7), followed by Biaffine (0.67) and StackPointer (0.64). The three of them also obtain a relatively high agreement with each other (0.7-0.85), in contrast to their agreements with others (0.47-0.66).
Among the parser pairs, CoreNLP and StackPointer obtain the lowest agreement of 0.47---we then observe that
all parsers achieve their lowest agreement with CoreNLP, compared to their agreements with other parsers
(0.47-0.56 vs. 0.53-0.85). Besides, we note that TowerParse also exhibits a relatively low agreement with others (0.5-0.66), especially with StackPointer (0.53) and CoreNLP (0.50).

As for \textbf{German} (Figure \ref{fig:parser_cor_de}), the highest agreements are observed between StackPointer and Biaffine, and between StackPointer and Stanza (0.77). Again, the lowest agreement is found between CoreNLP and StackPointer (0.45) and this low agreement with CoreNLP is consistent across parsers, ranging from 0.45 to 0.59. Similar to the observation on English data, %to the English data, 
Stanza achieves the highest average agreement (0.7), followed by Biaffine and StackPointer (0.67-0.68), and these three parsers %also
exhibit a higher level of agreement with each other (0.76-0.77), compared to their agreement with other parsers, which falls within the range of 0.45-0.67.
%obtain a slightly lower average agreement than Stanza 
. 

%again, Stanza has the highest average agreement (0.7), while CoreNLP obtains the lowest 
%average agreement 
%(0.5). 

In summary, our observations indicate that for both languages, \textbf{\emph{the use of different parsers may lead to various conclusions about the diachronic trend of syntactic change}}.
%the parsers do not always agree with each other.
%(1) Stanza exhibits the highest agreement with other parsers, while (2) CoreNLP demonstrates the lowest agreement; and (3) Biaffine, StackPointer, and Stanza agree with each other more than with other parsers. 
This raises some concerns about previous approaches %that conclude their findings 
with heavy reliance on the CoreNLP parser, which exhibits the lowest agreement with other parsers in our experiment.


%All parsers but CoreNLP show moderate to high agreement with each other. 


%show the correlation matrix between the parsers on each measure
%or maybe on the trend prediction

%emphasize the correlation of CoreNLP with others.


%\vspace{1cm}\noindent\textbf{RQ3: \emph{Do the measures show the same trend in English and German?}}



\vspace{1cm}\noindent\textbf{RQ3 \& RQ4: \emph{Which measures are decreasing/increasing over time? Do they show the same trend in English and German?}}\\

\noindent Recognizing that different parsers can lead to varying conclusions in trend tests, we employ a majority vote approach to identify the stable trends across parsers, i.e., if at least 3 out of 5 parsers agree on a trend, we consider it a stable trend. 
%This method aims to identify consistent trends across parsers. 
Besides, observing that the outcomes of the two trend tests often differ from each other, especially on the \texttt{Random} datasets, we further restrict the valid trends to those being consistent cross the two trend tests.


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[!ht]
\centering
\begin{subfigure}[]{\textwidth}
\resizebox{.95\linewidth}{!}{% 
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
measure              & all & 5  & 10 & 15 & 20 & 30 & 40 & 50 & 60 & 70 \\ \midrule
NDD                  &    & +5 & -5 & -5 &   &   &   &   &   &   \\
\underline{MDD}                  & -3  &   &   &   &   & -5 &   & -3 & -4 & -5 \\
\underline{Tree Height}               & +4  & -5 &   &   & +3 & +5 & +4 & +5 & +5 & +5 \\
\underline{\textbf{Left Children Ratio}}   & -4  & +4 &   &   & -4 & -5 & -4 & -3 & -5 & -5 \\
\underline{\textbf{Tree Degree}}               & -4  & +4 &   &   &   & -5 & -3 & -4 & -3 & -4 \\
\#Leaves          &    & +5 & +5 & +5 & +5 & +5 & +5 & +5 & +5 & +5 \\
Degree Variance          &    & +5 & +4 & +5 &   & -3 &   &   &   & -4 \\
\underline{Degree Mean}         & +3  &   & +4 & +4 & +5 & +5 & +5 & +5 & +5 & +5 \\
Topological Order Distance &    &   &   &   &   & +4 &   &   & +3 & +3 \\
Random Tree Distance &    &   &   &   &   &   &   &   &   &   \\
\underline{Root Distance}       & -5  & +4 & -5 & -5 &   &   &   &   &   &   \\
Longest Path Distance        &    &   &   &   &   &   &   &   &   &   \\
\underline{\textbf{\#Crossing}}        & -2   &   &   &   &   &   &   &   &   &   \\
\underline{Depth Variance}           & +4  & -4 &   &   & +3 & +5 & +4 & +5 & +5 & +5 \\
\underline{Depth Mean}          & +4  & -4 &   &   & +4 & +5 & +5 & +5 & +5 & +5 \\ \bottomrule
\end{tabular}%
}%
\caption{English}\label{tab:trend_en}
\end{subfigure}%

\begin{subfigure}[]{\textwidth}
\resizebox{.95\linewidth}{!}{% 
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
len\_group           & all & 5  & 10 & 15 & 20 & 30 & 40 & 50 & 60 & 70 \\ \midrule
\underline{NDD}                  & -5  & -5 & -5 &   & -3 & -5 &   &   &   &   \\ 
\underline{MDD}                  & +5  & +5 & +5 & +5 & +4 &   & +5 & +5 & +4 &   \\
Tree Height               &    & -5 &   &   &   & +4 &   &   & +3 & +3 \\
\underline{\textbf{Left Children Ratio}}   & -5  &   &   &   &   & -4 & -5 & -5 & -5 & -5 \\
\underline{\textbf{Tree Degree}}              & -4  & +5 & +5 &   & -4 & -4 & -5 & -5 & -5 & -5 \\
\underline{\#Leaves}          & -3  & +5 & +5 &   &   & -4 & -5 & -5 & -5 & -5 \\
\underline{Degree Variance}          & -4  & +5 & +5 &   & -4 & -4 & -5 & -5 & -5 & -5 \\
Degree Mean         &    &   & +5 &   &   &   & -3 & -3 & -4 & -4 \\
Topological Order Distance &    & -5 & -5 & -3 &   & +4 & +4 & +5 & +5 & +4 \\
Random Tree Distance &    &   &   &   &   &   &   &   &   &   \\
Root Distance       &    &   &   &   &   & -4 &   &   &   &   \\
\underline{Longest Path Distance}          & +3  & +5 & +5 & +3 &   & +4 & +5 & +5 & +4 & +3 \\
\underline{\textbf{\#Crossing}}        &  -2  &   &   &   &  -2 &   &   &   &   &   \\
Depth Variance           &    & -5 &   &   &   & +3 &   &   & +3 & +3 \\
Depth Mean          &    & -5 & -3 &   &   & +4 & +5 & +4 & +3 & +3 \\\arrayrulecolor{black}\bottomrule[1pt]
\end{tabular}%
}%
\caption{German}\label{tab:trend_de}
\end{subfigure}
\caption{Measures that have a stable trend across the two trend tests, supported by at least 3 parsers (except for ``\#Crossing'', for which we relax the minimal requirement to 2 parsers, as corenlp is unable to predict crossing edges.). ``$+$'' and ``$-$'' denote the increasing and decreasing trend respectively; the values refer to the number of parsers that agree with this trend. The measures that are stable in one language are underlined and those that show the same trend in English and German are bold.}
\label{tab:trend}
\end{table}

We demonstrate the results of the trend tests in Table \ref{tab:trend}, which shows the consistent trends across tests that are agreed by at least 3 parsers, except for \#Crossing, for which we relax the minimal requirement to 2 parsers, as CoreNLP can not predict the non-projective relations. ``$+$'' and ``$-$'' before the numbers denote the increasing and descreasing trend, repectively and the values after ``$+$/$-$'' refer to the number of parsers that support in this trend.

As shown in Table \ref{tab:trend}, on the \textbf{\texttt{Balance}} dataset: %we observe that:
 overall, (1) in \textbf{English}, we observe an \emph{increase} in the \emph{tree height}, \emph{degree mean}, \emph{depth mean} and \emph{depth variance} 
 %are \emph{increasing}
 over time, while the \emph{MDD}, \emph{left-children ratio}, \emph{tree degree}, \emph{root distance} and \emph{\#crossing} are \emph{decreasing};
 %over time; 
 (2) in \textbf{German}, the \emph{MDD}, \emph{longest path distance} are \emph{increasing} over time, whereas the \emph{NDD}, \emph{left-children ratio}, \emph{tree degree}, \emph{\#leaves}, \emph{degree variance}, and \emph{\#crossing} demonstrate a \emph{downward} trend. 
 
 We find three measures that show downtrend in both languages, i.e., the left-children ratio, tree degree, as well as the \#crossing. 
 All of the other measures show different trends across languages, including MDD, which has been shown to be decreasing over time in English in many domains. \todo{add citation}
%It is worth noting that in German, 
We also see a downward trend of MDD in English, especially for sentences of length greater than 30, where in 4 out of 5 length groups, 3-5 parsers support the decreasing trend. However, we do not see a clear clue about the trend in sentences of length smaller than 30. In contrast, we observe a consistent uptrend in MDD in German across different sentence lengths: in 7 out of 9 length groups, this trend is confirmed by at least 4 parsers. %As for NDD, we see an anti-minimization 

NDD, as the normalized version of MDD, is expected to demonstrate a consistent trend with MDD on the balanced dataset across sentence lengths; however, it suggests a totally opposite direction than MDD with respect to the language change in German, where MDD is increasing while NDD is decreasing over time. We note that in \citet{zhang2023investigation}, the MDD and NDD for the English news text also demonstrate inconsistent trends, where MDD is gradually increasing over time, while NDD does not show any clear trend. 
Those may cast doubts on the legitimacy of the NDD metric.

\todo{add examples for each measure}

%in the investigation of the language change in news text \citet{zhang2023investigation} also 
  

 %However, there is only little clue about the decreasing trend of MDD in German. 


%find the majority vote: trend consistent across parsers

%maybe select the best two parsers for each language? or maybe the agreed trend of parameters 

%include the trend parameters which show the strength of the trend 

%\vspace{1cm}\noindent\textbf{RQ5: What are the most influential parameters?}
%maybe show the correlation between the frequency of each relation type and the measures

==> structure_unused/6_discussion.tex <==
%\section{Discussion}

==> structure_unused/7_conclusion.tex <==
\section{Conclusion}

In conclusion, this study delved into diachronic language changes in English and German.
%, with a specific focus on syntactic dependency distance. 
We comprehensively examined 15 measures, including the mean dependency distance, across extensive corpora containing political debate texts. By analyzing the agreement among five different dependency parsers, including the commonly used Stanford CoreNLP, we provided novel insights into trends in language change.
Notably, we discovered a distinctive uptrend in the mean dependency distance in German, a trend consistent across various parsers and sentence lengths. Furthermore, three measures exhibited consistent trends across different parsers and languages, including a downward trend in left-children ratio, tree degree, and the number of crossing edges.
Our findings shed light on the dynamic nature of language evolution and the extent to which it may differ across languages. We emphasized the importance of considering various parsers in diachronic studies to avoid potential biases associated with parser-specific idiosyncrasies.
Additionally, this work demonstrated that the impact of data noise on parser performance was relatively minimal in the context of diachronic corpora. Parsers successfully navigated the challenges posed by older texts, enabling a deeper understanding of language change.
In essence, our research contributed to a more comprehensive understanding of the diachronic evolution of language and highlighted the need for multi-parser approaches in diachronic studies, thereby enriching our knowledge of how languages transformed over time.


\section{Ethical Concerns}

The authors of this paper freely used ChatGPT and Grammarly to rephrase the sentences and correct the grammar errors. 

==> structure_unused/8_ack.tex <==
\clearpage
\section{Acknowledgement}

\iffalse
I would like to greatly thank all the people who have helped me go through my Bachelor's and Master's studies in Germany.

First of all, I am extremely grateful to Dr. Steffen Eger for being my supervisor during the past two years. Without you, I would never have had a chance to start the academic journey that I could not have imagined previously. 

Secondly, I would like to thank my colleagues Buyuan Liu, Tianqi Luan and Yin Chen at TU Darmstadt. Without you, I could not even ``survive'' from the Bachelor's study.

Thirdly, I would like to thank my ``Animal Crossing'' family. Yuan Zang, Jia Chen, Chen Gong, Xinyi Yang, and Rongyuan Xu, you have provided me with very helpful emotional and mental support (and sometimes also financial support :)), which has made my life in Germany.

Lastly, I would like to thank my parents. You might not have always understood my choices, but you have given me full trust, support, and respect. 

\fi

==> tables/trendtable.tex <==
\begin{table}[!h]
\centering
\begin{subfigure}[]{\textwidth}
\resizebox{.95\linewidth}{!}{% 
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
len\_group           & all & 5  & 10 & 15 & 20 & 30 & 40 & 50 & 60 & 70 \\ \midrule
\underline{\mdd{}} & -3 & - & - & - & - & -4 & - & - & -3 & -4 \\ 
\ndd{} & - & +4 & -4 & -4 & - & - & - & - & - & - \\
\underline{\rootdis{}} & -5 & +4 & -5 & -5 & -3 & - & - & - & - & - \\
\underline{\height{}} & +4 & -5 & - & +3 & +4 & +5 & +4 & +5 & +5 & +5 \\
\underline{\depvar{}} & +4 & -5 & - & - & +4 & +5 & +4 & +5 & +5 & +5 \\
\underline{\depmean{}} & +4 & -5 & - & - & +5 & +5 & +5 & +5 & +5 & +5 \\
\underline{\degree{}} & -4 & +5 & - & - & - & -5 & -3 & -4 & -4 & -4 \\
\degvar{} & - & +5 & +3 & +5 & - & -4 & -3 & - & -3 & -5 \\
\underline{\degmean{}} & +3 & - & +5 & +5 & +5 & +5 & +5 & +5 & +5 & +5 \\
\underline{\headratio{}} & -4 & +4 & - & - & -4 & -5 & -5 & -4 & -5 & -5 \\
\headdis{} & - & - & - & - & +3 & +5 & +3 & +3 & +4 & +4 \\
\leaves & - & +5 & +5 & +5 & +5 & +5 & +5 & +5 & +5 & +5 \\
\underline{\crossing} & -2 & - & - & - & - & - & - & - & - & - \\
\lpath{} & - & - & - & - & - & - & - & - & - & - \\
\random{} & - & - & - & - & - & - & - & - & - & +3 \\ \bottomrule
\end{tabular}%
}%
\caption{English}\label{tab:trend_en}
\end{subfigure}%

\begin{subfigure}[]{\textwidth}
\resizebox{.95\linewidth}{!}{% 
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
len\_group           & all & 5  & 10 & 15 & 20 & 30 & 40 & 50 & 60 & 70 \\ \midrule
\underline{\mdd{}} & +5 & +5 & +5 & +5 & +4 & - & +5 & +5 & +4 & - \\
\underline{\ndd{}} & -5 & -5 & -5 & - & -3 & -5 & - & - & - & - \\
\rootdis{} & - & - & - & - & - & -4 & - & - & - & - \\
\height{} & - & -5 & - & - & - & +4 & - & - & +3 & +3 \\
\depvar{} & - & -5 & - & - & - & +3 & - & - & +3 & +3 \\
\depmean{} & - & -5 & -3 & - & - & +4 & +5 & +4 & +3 & +3 \\
\textbf{\underline{\degree{}}} & -4 & +5 & +5 & - & -4 & -4 & -5 & -5 & -5 & -5 \\
\underline{\degvar{}} & -4 & +5 & +5 & - & -4 & -4 & -5 & -5 & -5 & -5 \\
\degmean{} & - & - & +5 & - & - & - & -3 & -3 & -4 & -4 \\
\textbf{\underline{\headratio{}}} & -5 & - & - & - & - & -4 & -5 & -5 & -5 & -5 \\
\headdis{} & - & -5 & -5 & -3 & - & +4 & +4 & +5 & +5 & +4 \\
\underline{\leaves{}} & -3 & +5 & +5 & - & - & -4 & -5 & -5 & -5 & -5 \\
\textbf{\underline{\crossing{}}} & -2 & - & - & - & -2 & - & - & - & - & - \\
\underline{\lpath{}} & +3 & +5 & +5 & +3 & - & +4 & +5 & +5 & +4 & +3 \\
\random{} & - & - & - & - & - & - & - & - & - & - \\ \bottomrule
\end{tabular}%
}%
\caption{German}\label{tab:trend_de}
\end{subfigure}
\caption{Measures that have a stable trend across the two trend tests, supported by at least 3 parsers (except for ``\#Crossing'', for which we relax the minimal requirement to 2 parsers, as corenlp is unable to predict crossing edges.). ``$+$'' and ``$-$'' denote the increasing and decreasing trend respectively; the values refer to the number of parsers that agree with this trend. The \fix{overall} measures that are stable in one language are underlined and those that show the same trend in English and German are bold.}
\label{tab:trend}
\end{table}
